Adaptive Differentially Private Empirical Risk Minimization

We propose an adaptive (stochastic) gradient perturbation method for differentially private empirical risk minimization. At each iteration, the random noise added to the gradient is optimally adapted to the stepsize; we name this process adaptive differentially private (ADP) learning. Given the same privacy budget, we prove that the ADP method considerably improves the utility guarantee compared to the standard differentially private method in which vanilla random noise is added. Our method is particularly useful for gradient-based algorithms with time-varying learning rates, including variants of AdaGrad (Duchi et al., 2011). We provide extensive numerical experiments to demonstrate the effectiveness of the proposed adaptive differentially private algorithm.

==> 6paper-checklist.tex <==

\section*{Paper Checklist}

%\todo{\url{https://neurips.cc/Conferences/2021/PaperInformation/PaperChecklist}}



\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{As discussed in \cref{sec:future-work}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{This paper mainly focuses on theoretical analysis, and it does not have any negative social impact. }
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{As stated in the paper.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{All proofs are provided in the appendix (full paper).}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Code, data, and instructions can be found in the supplementary material (code).}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{As stated in \cref{sec:exp}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{As reported in \cref{table:cifar-decay} and \cref{table:cifar-adptive} in \cref{sec:exp}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{As stated in \cref{sec:exp} and the supplementary material (code).}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA {}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{The datasets are CIFAR10 and MNIST not containing personally identifiable information nor offensive content}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
\newpage

==> olds/adagrad-norm.tex <==


\subsection{DP-SGD with AdaGrad-Norm stepsize}\label{proof:adp-adagrad-norm1}
\begin{prop}(\textbf{DP-SGD with AdaGrad-Norm stepsize})\label{thm:dp-AdaGrad-Norm}
Set Algorithm 1 with $\alpha_{t+1}=1$, $b_{t+1}^2 =b_{t}^2+ \|\nabla f(\theta_{t};x_{\xi_t})+c_t\|^2$, and $\sigma = \frac{8G\log(1.25/\delta )}{  n \varepsilon }$ for some $T$.
The gradients follow 
\begin{footnotesize}
\begin{align}
   \min_{k\in{[T-1]}} \mathbb{E} [\|\nabla F(\theta_k)\|^2]
    &\leq G^2\left( \frac{2\sqrt{2}}{\sqrt{T}} + \frac{8d \sqrt{TB_\delta}}{n^2\varepsilon^2}\right)B_{\log} +G\sqrt{\frac{2}{T}+\frac{8dB_\delta }{n^2\varepsilon^2 } }\left(  \frac{ D_F }{\eta}+  \frac{\eta L}{2}B_{\log} 
 \right) \label{eq:adagrad-dp1}
\end{align}
\end{footnotesize}
where 
$B_\delta =8\log^2\left({1.25}/{\delta }\right)$ and $B_{\log} =  \log \left({T(G^2+d\sigma_z^2)}/{b_0^2} +1  \right)$.
\end{prop}

See the proof in Section \ref{proof:adp-adagrad-norm1}
Setting  $T = {n^2  \varepsilon^2 }/{64d\log^2(1.25/\delta )}$, we obtain the utility bound 
$U_{adagrad}=\mathcal{O}\left({G^2\sqrt{d\log(1/\delta )}\log(n/\delta )}/{(n\varepsilon)} \right)$



To be clear about the adaptive algorithm in Proposition \ref{thm:dp-AdaGrad-Norm}, we first state it in Algorithm \ref{alg:DP-AdaGrad-Norm} 
\begin{algorithm}[H]
\caption{\textbf{DP-SGD with AdaGrad-Norm stepsize }} \label{alg:DP-AdaGrad-Norm}
\begin{algorithmic}[1]
  \State {\bfseries Input:} 
   Initialize $x_0 \in \mathbb{R}^d, b_{0}>0, \eta>0$
    \For{\texttt{ $j = 1,2, \ldots$ }}
    
     %\State Generate  $\xi_{j-1}$ and $G_{j-1} = G(x_{j-1}; \xi_{j-1})$
     \State generate $\xi_t\sim \text{Uniform}(1,...,n)$  and $c_t\sim \mathcal{N}(0,\sigma I)$
      \State release gradient $G_t = \nabla F(\theta_{t};x_{\xi_t})+c_t$ 
      \State update ${b}_{t+1}^2 =  {b}_{t} ^2+ { \| G_{t} \|^2}$  
    %   \State $x_{j} = x_{j-1} -  \frac{\eta}{{b}_{j}}G_{j-1} $
	   % \State update $b_{t+1}$	 and $\alpha_{t+1}$ 

	   % \State $G_{t}= ,$ where
	    \State update $\theta_{t+1}=\theta_{t}-  \frac{\eta}{b_{t+1}}G_t$
	    \EndFor
\end{algorithmic}
  \end{algorithm}
% \begin{algorithm}[H]
% \caption{\textbf{DP-SGD with AdaGrad-Norm stepsize }}
% \label{alg:privacy-ada2}
% \begin{algorithmic}[1]
% 	    \State Input $\theta_0,b_t$,
% 	    \For {$ t=1,\ldots,T$} 
% 	      \State $\xi_t\sim \text{Uniform}(1,...,n)$  and $c_t\sim \mathcal{N}(0,\sigma I)$
% 	       \State release $G_{t}= \nabla L(\theta_{t};x_{\xi_t})+c_t,$ 
% 	       	    \State update  parameter $b^2_{t+1}=b^2_{t}+ \|G_t\|^2$
% 	    \State update gradient $\theta_{t+1}=\theta_{t}-\eta  \frac{1}{b_{t+1}}G_t$

% 	    \EndFor
% \end{algorithmic}
% \end{algorithm}
\begin{lemma}[AdaGrad-Norm \cite{ward2019adagrad}]\footnote{We are using Theorem 10 in this version \url{https://arxiv.org/pdf/1806.01811v5.pdf}  }
\label{thm:improveSGDmain}
Assume A1-A3. With $\sigma = 0$, the convergence in Algorithm~\ref{alg:DP-AdaGrad-Norm} follows,
\begin{align}
 \min_{\ell=0,1,\dots, T-1}  \mathbb{E}  [\|\nabla F(\theta_{\ell})\|^2]  \leq \left( \frac{2\sqrt{2}b_0}{T} + \frac{\sqrt{2}G}{\sqrt{T}}\right)\left(  \frac{ F_{0} - F^{*} }{\eta}+ \left(2{G} + \frac{\eta L}{2}\right) \log \left( \frac{TG^2}{b_0^2} +1  \right)
 \right)\label{eq:wu-bound}
\end{align}
\end{lemma}
For private AdaGrad-Norm, because the uniform sampling $\xi_k$ and the noise sampling $z_k$ are independent, we have that 
\begin{align}\mathbb{E}_{\xi_k}[ \mathbb{E}_{z_k}[ \|\nabla F(\theta_{\ell};x_{\xi_k}) +c_k\|^2]]= \mathbb{E}_{\xi_k}[ \|\nabla F(\theta_{\ell};x_{\xi_k})\|^2]+\mathbb{E}_{z_k}[ \|\vc_k\|^2]\leq  G^2+d\sigma^2;\end{align}
Replacing $G$ in inequality \ref{eq:wu-bound} with $\sqrt{G^2+d\sigma^2}$ and setting $B_{\log} =  \log \left( \frac{T(G^2+d\sigma^2)}{b_0^2} +1  \right)$
, we have the convergence bound of Algorithm \ref{alg:DF-AdaGrad-Norm} \todo{missing ref}
\begin{align}
 \min_{\ell=0,1,\dots, T-1} \left( \mathbb{E}  \|\nabla F(\theta_{\ell})\|^{
   \frac{4}{3}} \right)^\frac{3}{2}  
   &\leq \left( \frac{2\sqrt{2}b_0}{T} + \frac{\sqrt{2}\sqrt{G^2+d\sigma^2}}{\sqrt{T}}\right)\left(  \frac{ F_{0} - F^{*} }{\eta}+ \left(2\sqrt{G^2+d\sigma^2} + \frac{\eta L}{2}\right)B_{\log} 
 \right) \nonumber\\
&\overset{(a)}{\leq} \left(  \frac{2\sqrt{2}\sqrt{G^2+d\sigma^2}}{\sqrt{T}}\right)\left(  \frac{ F_{0} - F^{*} }{\eta}+ \left(2\sqrt{G^2+d\sigma^2} + \frac{\eta L}{2}\right)B_{\log} 
 \right) \label{eq:wu-bound1}
 \\
   & \overset{(b)}{=} \frac{G\sqrt{dB_\delta}}{n\varepsilon_{SGD}} \left(\frac{ F_{0} - F^{*} }{\eta}+ \frac{\eta L}{2}B_{\log} \right)+     \frac{32G^2\sqrt{dB_\delta}}{ n \varepsilon_{SGD}}  B_{\log}
%  \nonumber\\
%   &\leq 
\end{align}
where (a) is due to the condition that $T\geq 4b_0^2/(G^2+d\sigma^2)$; (b) follows by setting $T = \frac{n^2  \varepsilon^2_{SGD}}{64d\log(1.25/\delta_{SGD})}$ and $B_\delta =8\log \left(\frac{n  \varepsilon^2_{SGD} }{d\delta_{SGD}\log(\frac{1.25}{\delta_{SGD}})}\right)\log\left(\frac{1.25}{\delta_{SGD}}\right)$.  The way we chose $T$ is according to 
\begin{align}
   \frac{G^2+d\sigma^2}{T} =\frac{G^2}{T}+ \frac{64dG^2\log(T/(n\delta_{SGD})\log(1.25/\delta_{SGD})}{ n^2 \varepsilon^2_{SGD}} \overset{(a)}{\geq } \frac{16G^2\sqrt{d\log(T/(n\delta_{SGD})\log(1.25/\delta_{SGD})}}{ n \varepsilon_{SGD}\sqrt{T}} 
\end{align}
where the equality in (a) holds when $G^2 = d\sigma^2$. 

==> olds/backup-privacy-gurantee.tex <==

\section{Privacy Guarantee for Algorithm  \ref{alg:privacy-ada1} (version 2)}
\begin{prop}\label{def:privacy-ada1}
Let $Z\sim\mathcal{N}(0,\sigma_z^2)$. At iteration $t$, we have the privacy mechanism $\mathcal{M}_t:\mathbb{R}^d\to\mathbb{R}^d$ for $f_t(X)=\nabla L(\theta_t;x_{\xi_t})$  with $x_{\xi_t}\sim X$ :
%some $f(X):\mathbb{R}\to\mathbb{R}$ and $b(X):\mathbb{R}\to\mathbb{R}$ follows
\[\mathcal{M}^{\text{AG}}_t(X)=\frac{f_t(X)}{\sqrt{b_t^2(X)+\|f_t(X)\|^2}}+Z\]
where   $b^2(X) = b_0^2+\sum_{k=1}^{t-1}\| \nabla L(\theta_k;x_{\xi_k})\|^2$ for Algorithm \ref{alg:privacy-ada1} and  $b^2(X) = b_0^2+\sum_{k=1}^{t-1}\| \nabla L(\theta_k;x_{\xi_k})\|^2+\varepsilon \|c_t\|^2$ for Algorithm \ref{alg:privacy-ada2}

\end{prop}
The proof of the proposition is straight forward for the above mechanism for Algorithm \ref{alg:privacy-ada1} at iteration $t$.

Define the distance $\Delta_t^{\text{AG}} = \left\| \frac{f_t(X)}{\sqrt{b_t^2(X)+\|f_t(X)\|^2}}- \frac{f_t(X')}{\sqrt{b_t^2(X')+\|f_t(X')\|^2}} \right\|^2$. % \|\frac{f_t(X)}{\sqrt{b_t^2(X)+f_t^2(X)}}-\frac{f_t(X')}{\sqrt{b_t^2(X')+\|f_t(X')\|^2}}\|^2$ 
The upper bound of  $\Delta_t^{\text{AG}}$ is % the the norm different between $M(X)$ and $M(X')$
\begin{align}
 \Delta^{\text{AG}}_t 
      %&= \left\| \frac{f_t(X)}{\sqrt{b_t^2(X)+\|f_t(X)\|^2}}- \frac{f_t(X')}{\sqrt{b_t^2(X')+\|f_t(X')\|^2}} \right\|_2^2 \\
    %   &\leq 2\left\| \frac{f_t(X)}{\sqrt{b_t^2(X)+f_t^2(X)}}\right\|^2+\left\| \frac{f_t(X')}{\sqrt{b_t^2(X')+\|f_t(X')\|^2}} \right\|^2 \\
              &\leq\frac{ 2\left\| f_t(X)\right\|^2}{{b_t^2(X)+\|f_t(X)\|^2}}+ \frac{2\left\|f_t(X')\right\|^2}{{b_t^2(X')+\|f_t(X')\|^2}}  %\\
            %   &\leq \left\| \frac{G}{\sqrt{b_t^2(X)+G^2}}\right\|+\left\| \frac{G'}{\sqrt{b_t^2(X')+G'^2}} \right\|_2 \\
\end{align}
The supreme of $\Delta_t^{\text{AG}}$ and $ \sum_{t=0}^{T-1}\Delta_t^{\text{AG}}$ over the iterations ${f_t(X)}$ and ${f_t(X)}$ is
\begin{align}
\sup_{t,X,X'} \Delta^{\text{AG}}_t 
              &\leq \sup_{t,X,X'} \frac{ 2\left\| f_t(X)\right\|^2}{{b_t^2(X)+\|f_t(X)\|^2}}+ \sup_{t,X,X'}\frac{2\left\|f_t(X')\right\|^2}{{b_t^2(X')+\|f_t(X')\|^2}} \leq \frac{ 4G^2}{{b_0^2+G^2}}  \label{eq:adagrad-one}
\end{align}
The sum of $\Delta_t^{\text{AG}}$ from $t=0$ to $t=T-1$ is
\begin{align}
 \sum_{t=0}^{T-1}\Delta_t^{\text{AG}}
      %&= \left\| \frac{f_t(X)}{\sqrt{b_t^2(X)+\|f_t(X)\|^2}}- \frac{f_t(X')}{\sqrt{b_t^2(X')+\|f_t(X')\|^2}} \right\|_2^2 \\
    %   &\leq 2\left\| \frac{f_t(X)}{\sqrt{b_t^2(X)+\|f_t(X)\|^2}}\right\|^2+\left\| \frac{f_t(X')}{\sqrt{b_t^2(X')+\|f_t(X')\|^2}} \right\|^2 \\
              &\leq \sum_{t=0}^{T-1}\frac{ 2\left\| f_t(X)\right\|^2}{{b_t^2(X)+\|f_t(X)\|^2}}+ \sum_{t=0}^{T-1}\frac{2\left\|f_t(X')\right\|^2}{{b_t^2(X')+\|f_t(X')\|^2}}  \\
               &\leq \sum_{t=0}^{T-1}\frac{ 2\left\| f_t(X)\right\|^2}{{b_0^2+\sum_{k=0}^t\|f_k(X)\|^2}}+ \sum_{t=0}^{T-1}\frac{2\left\|f_t(X')\right\|^2}{{b_0^2+\sum_{k=0}^t\|f_k(X')\|^2}}  \\
            &\leq 4+2\log\left(1+b_0^2+\sum_{t=0}^{T-1}\left\| f_t(X)\right\|^2 \right)+ 2\log\left(1+b_0^2+\sum_{t=0}^{T-1} \left\| f_t(X')\right\|^2 \right) 
            %   &\leq \left\| \frac{G}{\sqrt{b_t^2(X)+G^2}}\right\|+\left\| \frac{G'}{\sqrt{b_t^2(X')+G'^2}} \right\|_2 \\
\end{align}
Note that we assume $ \sup_{t, X}\|{f_t(X)}\|\leq G$ uniform bounded for any $X$.
Thus the supreme of  $ \sum_{t=0}^{T-1}\Delta_t^{\text{AG}}$ over the iterations ${f_t(X)}$ and ${f_t(X)}$ is
% \begin{align}
% \sup_{t,X,X'} \Delta^{\text{AG}}_t 
%               &\leq \sup_{t,X,X'} \frac{ 2\left\| f_t(X)\right\|^2}{{b_t^2(X)+\|f_t(X)\|^2}}+ \sup_{t,X,X'}\frac{2\left\|f_t(X')\right\|^2}{{b_t^2(X')+\|f_t(X')\|^2}} \leq \frac{ 4G^2}{{b_0^2+G^2}}  \label{eq:adagrad-one}
% \end{align}
\begin{align}
\sup_{t,X,X'} \sum_{t=0}^{T-1}\Delta_t^{\text{AG}}
            &\leq 4+2\log\left(1+b_0^2+\sup_{t,X,X'} \sum_{t=0}^{T-1}\left\| f_t(X)\right\|^2 \right)+ 2\log\left(1+b_0^2+\sup_{t,X,X'}\sum_{t=0}^{T-1} \left\| f_t(X')\right\|^2 \right)\label{eq:adagrad-T}\\
      &\leq 4+4\log\left(1+b_0^2+TG^2 \right)
      %\\
            %   &\leq \left\| \frac{G}{\sqrt{b_t^2(X)+G^2}}\right\|+\left\| \frac{G'}{\sqrt{b_t^2(X')+G'^2}} \right\|_2 \\
\end{align}
Some high-level thought for Algorithm 1 (SGD with Gaussian Mechanism) $\mathcal{M}_t^{\text{GD}} = f_t(X)+Z$. Denote each step $ \Delta^{\text{GD}}_t= \|\nabla f_t(X)-f_t(X')\|^2$ and so
\[\sup_{w,X,X'}\Delta^{\text{GD}}_t\leq 4G^2 \text{ and } \sup_{t,X,X'} \sum_{t=0}^{T-1}\Delta_t^{\text{GD}}\leq 4TG^2\] 
Thus the random variable $\theta_T$ for the final iterations $T$ is 
\begin{align}
    \theta_T &= \theta_{T-1} - \eta \nabla L(\theta_{T-1};X)+ Z \\
    &=   \theta_0 -\sum_{t=0}^{T-1}\left( \nabla  L(\theta_t;X)+ Z\right)\\
    &=  \theta_0 - \eta \sum_{t=0}^{T-1}\nabla  L(\theta_t;X) - \eta T Z 
    %\text{ and }    \theta'_T = \theta_0 - \eta   \sum_{t=0}^{T-1} \left( \nabla L(\theta'_t;X') + Z\right)
\end{align}
One might think of this $\theta_T$ is  applied by Gaussian Mechanism. According to Definition \ref{def:gaussian}, as we that $h(X) = \sum_{t=0}^{T-1}\nabla  L(\theta_t;X) $ and so $\sigma_{GD-T}^2 = T\sigma_z^2$, \me{this is not exactly right, since $\theta_t$ is affected by previous Gaussian... But I believe with some condition probability proof, we can come with some similar one.}  we have 
\[\sup_{X,X}\|h(X)-h(X')\|= \sup_{X,X'}\left\| \sum_{t=0}^{T-1} \left(\nabla  L(\theta_t;X)-\nabla  L(\theta_t;X')\right)\right\|\]

The difference between $\theta_T$ and $\theta_T'$





==> olds/backup.tex <==
\section{Privacy Guarantee for Algorithm \ref{alg:privacy1} (version 2)}
\begin{prop}
Let $Z\sim\mathcal{N}(0,\sigma_z^2)$. At iteration $t$, we have the privacy mechanism $\mathcal{M}_t:\mathbb{R}^d\to\mathbb{R}^d$ for $f_t(X)=\nabla L(\theta_t;x_{\xi_t})$  with $x_{\xi_t}\sim X$ :
%some $f(X):\mathbb{R}\to\mathbb{R}$ and $b(X):\mathbb{R}\to\mathbb{R}$ follows
\[\mathcal{M}^{\text{SGD}}_t(X)=\frac{f_t(X)}{\sqrt{b_0+tc_b}}+Z.\]
\end{prop}

Define the distance $\Delta_t^{\text{SGD}} = \left\| \frac{f_t(X')-f_t(X)}{\sqrt{b_t^2+tc_b}} \right\|^2$. % \|\frac{f_t(X)}{\sqrt{b_t^2(X)+f_t^2(X)}}-\frac{f_t(X')}{\sqrt{b_t^2(X')+\|f_t(X')\|^2}}\|^2$ 
The upper bound of  $\Delta_t^{\text{AG}}$ is % the the norm different between $M(X)$ and $M(X')$
\begin{align}
 \Delta^{\text{SGD}}_t 
  &\leq\frac{ \left\|f_t(X')-f_t(X)\right\|^2}{\sqrt{b_0^2+tc_b}}
\end{align}
The supreme of $\Delta_t^{\text{SGD}}$  over the iterations ${f_t(X)}$ and ${f_t(X)}$ is
\begin{align}
\sup_{X,X'} \Delta^{\text{SGD}}_t \leq \frac{G^2}{\sqrt{b_0^2+tc_b}}
\end{align}
Thus, by Lemma \ref{lem:gaussian} and  privacy by amplification, $\mathcal{M}_t^{\text{AG}}$ at $t$ iteration is $(\varepsilon_t, \delta_t)-$DP if  $Z\sim \mathcal{N}(0,\sigma_z)$ where
\begin{align}
  \varepsilon_t  \leq \frac{ \sqrt{2\ln(1.25/\delta_t)}}{ n\sigma_z}\sqrt{\frac{ G^2}{{b_0^2+t c_b}} } 
\end{align}
Let $\delta_0=\delta_2=\ldots=\delta_t$. Using  extended advanced composition \ref{thm:advanced-comp}, we have the final output follow $(\varepsilon_{SGD}, \delta_{\text{SGD}})-DP$ where 

 \begin{align}
   \varepsilon_{SGD} &= \sqrt{\sum_{t=0}^{T-1} \varepsilon_t^2 \log\left(\frac{1}{\delta'}\right)} +  \sum_{i=1}^K \frac{\varepsilon_t^2}{2+\varepsilon_t} \\
   &\leq 2\sqrt{\sum_{t=0}^{T-1} \varepsilon_t^2 \log\left(\frac{1}{\delta'}\right)}\\
   &\leq \frac{2\sqrt{2\log\left({1}/{\delta'}\right)\log\left({1.25}/{\delta_0}\right)}}{n  \sigma_z} \sqrt{\sum_{t=1}^{T-1}  \frac{ G^2}{b_0+t c_b}  }      \\
   &= \frac{2G\sqrt{2\log\left({1}/{\delta'}\right)\log\left({1.25}/{\delta_0}\right)}}{n \sigma_z} \sqrt{\frac{ 1}{c_b}\sum_{t=1}^{T-1}  \frac{1}{b_0/c_b+t} }    \\
      &\leq \frac{2G\sqrt{2\log\left({1}/{\delta'}\right)\log\left({1.25}/{\delta_0}\right)}}{n \sigma_z} \sqrt{\frac{1}{b_0}+\frac{1}{c_b}\log \left(\frac{b_0+Tc_b}{b_0}\right)}  \\
  &= \mathcal{O}\left( \frac{G\sqrt{\log\left({1}/{\delta'}\right)\log\left({1}/{\delta_0}\right)}}{n \sigma_z} \sqrt{\frac{1}{b_0}+\frac{\log(1+Tc_b/b_0)}{c_b}}     \right)
\end{align}
Here, in the first inequality, the term $\sum_{i=1}^K \frac{\varepsilon_t^2}{2+\varepsilon_t}$ is considerable smaller  than $\sqrt{\sum_{t=0}^{T-1} \varepsilon_t^2 \log\left(\frac{1}{\delta_0}\right)}$. In addition,
\begin{align}
\delta_{\text{SGD}} &= 1 - (1- \delta_0) (1- \delta_1)(1-\delta_2) \hdots (1-\delta_{T-1}) + \delta' 
   = 1 - (1- \delta_0)^T + \delta' \leq \delta'
\end{align}
This implies that 
\begin{align}
    \varepsilon_{SGD} = \mathcal{O}\left( \frac{G\sqrt{\log\left({1}/\delta_{\text{SGD}}\right)\log\left({1}/{\delta_0}\right)}}{n \sigma_z} \sqrt{\frac{\log(T)}{c_b}}     \right)
\end{align}


\begin{align}
    \varepsilon_{SGD} = \mathcal{O}\left( \frac{G \log\left({1}/{\delta_{SGD}}\right)}{n \sigma_z} \sqrt{\frac{\log(T)}{c_b}}     \right)
\end{align}
\subsection{Convergence}
Assume
\begin{enumerate}
\item[A1] The random vectors $\xi_k$, $k = 0,1,2, \dots, $ are independent of each other and also of $x_k$;
% \item[A2] $\mathbb{E}_{\xi_k}[ \| G(x_k, \xi_k) -\nabla F(x_k) \|^2] \leq \sigma_G^2;$
\item[A2] $\| \nabla F(x) \|^2 \leq G^2$ uniformly.
\end{enumerate}
Recall the update in Algorithm \ref{alg:privacy-ada2}:
\begin{align*}
\theta_{t+1}&= \theta_t - \eta \frac{\eta g_{\xi_t}}{\sqrt{b^2_{0}+ tc_b}}+ \eta Z
\end{align*}
By Lipschitz gradient smoothness:
\begin{align}
L(\theta_{j+1}) &\leq L(\theta_{j}) - \eta\langle{ \nabla L(\theta_j),\frac{ g_{\xi_j}}{\sqrt{b^2_{0}+ tc_b}} +z_j\rangle}+\frac{ \eta^2 L}{2} \left\| \frac{ g_{\xi_j}}{\sqrt{b^2_{0}+ tc_b}}+  z_j  \right\|^2 \nonumber \\
\mathbb{E}[L(\theta_{j+1})] &\leq \mathbb{E}[L(\theta_{j})] -\frac{ \eta \mathbb{E}[\|\nabla L(\theta_{j})\|^2]}{\sqrt{b^2_{0}+ tc_b}} +\frac{ \eta ^2 L}{2(b_{0}+ tc_b)} \mathbb{E}[\|g_{\xi_j}\|^2]  +\frac{ \eta ^2 d L \sigma_z^2}{2} % \label{remark2}
\end{align}
So we have%think about $\eta_t = \frac{\eta}{\sqrt{b^2_{0}+ tc_b}}$
\begin{align*}
 \frac{ 1}{\sqrt{b_0^2+ Tc_b}} \sum_{\ell=0}^{T-1}\mathbb{E}  \|\nabla L(\theta_\ell)\|^2
   & \leq \sum_{\ell=0}^{T-1}\frac{\mathbb{E}  \|\nabla L(\theta_\ell)\|^2}{\sqrt{b_0^2+\ell c_b}} 
    \leq  \frac{\mathbb{E}[L(\theta_{0})]  }{\eta}+ \frac{\eta G^2 L}{2}\sum_{\ell=0}^{T-1} \frac{1}{b_0+ tc_b}  +\frac{ \eta dT L \sigma_z^2}{2}  \\
   \Rightarrow \frac{1}{T}\sum_{\ell=0}^{T-1}\mathbb{E}  \|\nabla L(\theta_\ell)\|^2
   & \leq  \frac{\sqrt{b_0^2+ Tc_b}\mathbb{E}[L(\theta_{0})]  }{T \eta}+ \frac{\eta G^2 L\sqrt{b_0^2+ Tc_b}}{2b_0T}\left(1+\frac{b_0\log(1+Tc_b/b_0)}{c_b}\right)  +\frac{ \eta d\sqrt{b_0^2+ Tc_b} L \sigma_z^2}{2}  \\
   & =\mathcal{O}\left(\frac{\sqrt{c_b}}{ \eta \sqrt{T}}\right) + \mathcal{O}\left(\frac{\eta G^2 L\log(1+Tc_b/b_0)}{ \sqrt{Tc_b}}\right)  +\frac{ \eta d\sqrt{b_0^2+ Tc_b} L}{2} \frac{G^2 \log^2\left({1}/{\delta_{SGD}}\right)}{n^2 \varepsilon^2_{SGD}} \frac{\log(T)}{c_b}   \\   
\end{align*}
% \begin{remark}
% Compare with Standard SGD

% % $\eta =\mathcal{O} \left(\frac{1}{\sqrt{t}}\right)$


% \end{remar

==> olds/basics.tex <==

\section{Revisit Differential Privacy of Stochastic Gradient Descent}\label{sec:privacy}
\begin{defn}
Let $\mathcal{D}$ be a collection of datasets. Two datasets $D$ and $D'$ are adjacent if they differ in at most one user data. A mechanism
$\mathcal{M}: \mathcal{D} \rightarrow \mathcal{R}$ with domain $\mathcal{D}$
and range $\mathcal{R}$ is $(\epsilon,\delta)$-differentially private if for 
any two adjacent datasets $D, D' \in \mathcal{D}$ and for any subset of outputs $S \subseteq \mathcal{R}$,
\[
\text{Pr} [\mathcal{M}(D) \in S ] \le e^{\epsilon} \text{Pr} [\mathcal{M}(D') \in S] + \delta.
\]
\end{defn}
% $b_{t+1}=1$

%For stochastic gradient descent,  we use Gaussian Mechanism or Laplace Mechanism to protect the privacy:
\begin{minipage}[t]{0.5\textwidth}
\begin{algorithm}[H]
\caption{\textbf{Private SGD}}
\label{alg:privacy}
\begin{algorithmic}[1]
	    \State Input $\theta_0$
	    \For {$ t=1,\ldots,T$} 
	    \State $\theta_{t+1} = \theta_{t}-\eta \left(\nabla L(\theta_{t};x_{\xi_t})+c_t\right), $  where
	    
	    $\xi_t\sim \text{Uniform}(1,...,n)$  and $c_t\sim \mathcal{N}(0,\sigma_t I)$
	    \EndFor
\end{algorithmic}
\end{algorithm}
\end{minipage}


\begin{minipage}[t]{0.5\textwidth}
\begin{algorithm}[H]
\caption{\textbf{Private SGD} (version 2)}
\label{alg:privacy1}
\begin{algorithmic}[1]
	   % \State Input $\theta_0$
	   % \For {$ t=1,\ldots,T$} 
	   % \State $\theta_{t+1} = \theta_{t}-\frac{\eta \nabla L(\theta_{t};x_{\xi_t})}{\sqrt{tc_b+b_0}}+\eta c_t, $  where
	   % $\xi_t\sim \text{Uniform}(1,...,n)$  and $c_t\sim \mathcal{N}(0,\sigma_t I)$
	   % \EndFor
	    \State Input $\theta_0,b_t$,
	    \For {$ t=1,\ldots,T$} 
	      \State $\xi_t\sim \text{Uniform}(1,...,n)$  and $c_t\sim \mathcal{N}(0,\sigma I)$
	    \State update $b^2_{t+1}=b^2_{t}+c_b$	    
	    \State $G_{t}= \nabla L(\theta_{t};x_{\xi_t})+b_{t+1}c_t,$ where
	    \State update $\theta_{t+1}=\theta_{t}-\eta  \frac{1}{b_{t+1}}G_t$
	    \EndFor
\end{algorithmic}
\end{algorithm}
\end{minipage}
\begin{minipage}[t]{0.5\textwidth}
\begin{algorithm}[H]
\caption{\textbf{Private AdaGrad-Norm} (version 3)}
\label{alg:privacy-ada2}
\begin{algorithmic}[1]
	    \State Input $\theta_0,b_t$,
	    \For {$ t=1,\ldots,T$} 
	      \State $\xi_t\sim \text{Uniform}(1,...,n)$  and $c_t\sim \mathcal{N}(0,\sigma I)$
	    \State update $b^2_{t+1}=b^2_{t}+\max{\{\|\nabla L(\theta_{t};x_{\xi_t})\|^2,c_b\}}$	    
	    \State $G_{t}= \nabla L(\theta_{t};x_{\xi_t})+b_{t+1}c_t,$ where
	    \State update $\theta_{t+1}=\theta_{t}-\eta  \frac{1}{b_{t+1}}G_t$
	    \EndFor
\end{algorithmic}
\end{algorithm}
\end{minipage}





% \begin{minipage}[t]{0.5\textwidth}
% \begin{algorithm}[H]
% \caption{\textbf{Private AdaGrad-Norm} (version 2)}
% \label{alg:privacy-ada1}
% \begin{algorithmic}[1]
% 	    \State Input $\theta_0,b_t$,
% 	    \For {$ t=1,\ldots,T$} 
% 	    \State update $b^2_{t+1}=b^2_{t}+\|\nabla L(\theta_{t};x_{\xi_t})\|^2$	    
% 	    \State $G_{t}= \nabla L(\theta_{t};x_{\xi_t})+b_{t+1}c_t,$ where
	    
% 	    $\xi_t\sim \text{Uniform}(1,...,n)$  and $c_t\sim \mathcal{N}(0,\sigma I)$

% 	    \State update $\theta_{t+1}=\theta_{t}-\eta  \frac{1}{b_{t+1}}G_t$
% 	    \EndFor
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}


\begin{minipage}[t]{0.5\textwidth}
\begin{algorithm}[H]
\caption{\textbf{Private $\beta$-AdaGrad-Norm }}
\label{alg:privacy-ada3}
\begin{algorithmic}[1]
	    \State Input $\theta_0,b_t$,
	    \For {$ t=1,\ldots,T$}
	    \State update  $(b^{\beta}_{t+1})^2=\beta b^2_{t}+\|G_t\|^2$
	    \State $G_{t}= \nabla L(\theta_{t};x_{\xi_t})+c_t,$  where
	    
	    $ \xi_t\sim \text{Uniform}(1,...,n)$  and $c_t\sim \mathcal{N}(0,\sigma I)$

	    \State update  $\theta_{t+1}=\theta_{t}-\frac{\eta}{{b^\beta_{t+1}}}G_t$
	    \EndFor
\end{algorithmic}
\end{algorithm}
\end{minipage}
\begin{minipage}[t]{0.5\textwidth}
\begin{algorithm}[H]
\caption{\textbf{SAGD \cite{zhou2020towards}}}
\label{alg:privacy-ada4}
\begin{algorithmic}[1]
	    \State Input $\theta_0,b_t$,
	    \For {$ t=1,\ldots,T$}
	    \State update $[b_{t+1}^2]_i=(1-\beta)\sum_{i=1}^t\beta [\nabla L^2(\theta_{t};x_{\xi_t})]_i$
	    \State $G_{t}=\nabla L(\theta_{t};x_{\xi_t})+c_t,$
	    
	    $ \xi_t\sim \text{Uniform}(1,...,n)$  and $c_t\sim \mathcal{N}(0,\sigma I)$
	    \State update $[\theta_{t+1}]_i=[\theta_{t}]_i-\frac{\eta}{[b_{t+1}]_i}[G_t]_i$
	    \EndFor
\end{algorithmic}
\end{algorithm}
\end{minipage}
Add the algorithm
% \begin{algorithm}[H]
% \caption{\textbf{Private SignSGD}(an extension of SignSGD \cite{bernstein2018signsgd})}
% \label{alg:privacy-ada}
% \begin{algorithmic}[1]
% 	    \State Input $\theta_0,b_t$,
% 	    \For {$ t=1,\ldots,T$} 
% 	    \State $G_t= n  \text{sign}(\nabla L(\theta_{t-1};x_{\xi_t})+c_t, \quad \xi_t\sim \text{Uniform}(1,...,n)$  and $c_t\sim \mathcal{N}(0,\sigma I)$
% 	    \State update $\theta_t=\theta_{t-1}-\eta G_t$
% 	    \EndFor
% \end{algorithmic}
% \end{algorithm}
% \[w_{t+1}=w_{t+1}-\frac{1}{b_t}g_t\]
% \[E|f(w_T;z)|+E|f(w_T';z)|<E|f(w_{T-1};z)|+\frac{1}{T}+E|f(w_{T-1}';z)|+\frac{1}{T} \]
%  $\sum_{t=1}^T\sqrt{\frac{1}{t}}$
%  $b_{t}=\mathcal{O}\left({\sqrt{T}}\right)$

\vspace{0.3cm}

 $b_t=(1+t)^{1/2}$
Without $c_t$, we know the convergence of \textbf{Algorithm 1} for convex smooth function with learning rate $\eta_t = \frac{1}{G\sqrt{t}}$, $\sigma_t=\sigma$ and $G=nL$. 

\begin{align}
    \mathbb{E}[L(\theta_T)]-L^*=\mathcal{O}\left( \frac{G\log(T)}{\sqrt{T}}\right) 
\end{align}
As we care about the information privacy, we would like to know the Differential Privacy as well as the convergence  (utilities) when analysing \textbf{Algorithm \ref{alg:privacy}}.
% A simple analysis would be: (1) Suppose each step, we have $(\varepsilon_0, \delta_0)$-DP. (2) After $T$ step, by advanced composition theorem, the algorithm
% $$(\epsilon \sqrt{T(1/\delta)}, \delta T)-\text{DP}.$$ {\color{blue}{This would be too bad, then $T=\mathcal{O}(1)$}.} The algorithm will not converge at all if we want to have good privacy. 
The analysis of the Algorithm 1 follows three steps (Based on \cite{kasiviswanathan2011can,song2013stochastic,bassily2014private}):
\begin{itemize}
    \item[1.] Suppose the gradient sensitivity of the loss function is $\sup_{w,X,X'} \|\nabla L(w;X)-\nabla L(w;X')\|\leq 2G$ for some positive constant $G$. We decide the privacy mechanism, for instance Gaussian Mechanism $\mathcal{M}$. Using Algorithm 1, we need to set $\sigma = \frac{2 ( 2G)\sqrt{\log(1/\delta)}}{\varepsilon}$ \cite{gautam2020}. % or Laplace Mechanism;  The privacy loss (random variable) with $1-\frac{\delta}{2}$ \[\|G(\theta_t)\|=\|n\left(\nabla L(\theta_{t}; z_i)+b_t\right)\|\leq \frac{d\epsilon}{2\sqrt{\log(1/\delta)}}, \forall t\]
    \begin{defn}\label{def:gaussian} 
    Let $h: \mathcal{X}^n \to \mathbb{R}^d$. The Gaussian mechanism is defined as
$\mathcal{M}(X) = h(X) + [[Z]_1, . . . , [Z]_k]^\top$,
where the $[Z]_i, i = 1,\ldots,k$ are independent $\mathcal{N}(0, \sigma_z^2
)$ random variables.
    \end{defn}
    \begin{lemma}\label{lem:gaussian} 
    The Gaussian mechanism is $(\varepsilon, \delta)$-differentially private if $\sigma_z = \sqrt{2\ln(1.25/\delta)}\Delta/\varepsilon$ where $\Delta = \sup_{X,X'} \|h(X)-h(X') \|$.
    \end{lemma}
    \item[2.] We decide the sampling, for instance, uniform sampling (line 3 in Algorithm 1) or others. We could apply amplification by sub-sample \cite{kasiviswanathan2011can}:
    \begin{lemma}
    Let the mechanism $\mathcal{M}:\mathcal{D}\to \mathcal{R}$ be $(\varepsilon,\delta)$-DP. Consider $\mathcal{M}_q$ follows the two steps (1) sample a random $q$ fraction of $\mathcal{D}$ (2) run $\mathcal{M}$ on the sample.
   Then the mechanism $\mathcal{M}_q$ is $(2q\varepsilon, q\delta)$-DP.
    \end{lemma}
Thus each step in Algorithm 1, we have $(\frac{\varepsilon}{n},\frac{\delta}{n})-DP$
   \item[3.] By advanced composition (Theorem III.3 \cite{dwork2010boosting}\footnote{If $\mathcal{M}_1,\mathcal{M}_2,...\mathcal{M}_k$ are $(\epsilon_0,\delta_0)-DP$, then $\mathcal{M}_{1:k}$ is $(\varepsilon,k\delta_0+\delta)-DP$ for $\varepsilon=\varepsilon_0\sqrt{2k \log(1/\delta)}+k\varepsilon_0 (exp(\varepsilon_0-1))$}  or Theorem 3.20 in \cite{dwork2014algorithmic})after $T$ step, Algorithm 1 would follow
   $$(\varepsilon \frac{\sqrt{T\log(1/\delta)}}{n}, \frac{\delta T}{n})-\text{DP}.$$ 
   
      $$\left( \frac{4G\log(1/\delta)\sqrt{T}}{  n\sigma_z }, \frac{\delta T}{n}\right)-\text{DP}.$$ 
      
            $$\left( \frac{2G\log(1/\delta)\sqrt{t}}{  n\sigma_z }, \frac{\delta T}{n}\right)-\text{DP}.$$ 
      
   We thus can decide $T=n^2$ and  have both of the worlds (privacy and convergence).
\end{itemize}
 

\subsection{Research questions:} 
\begin{itemize}
                                                                       
    \item[(1)] We could directly use the above techniques (step 1,2 and 3) to understand private adaptive gradient methods (see Algorithm \ref{alg:privacy-ada}). This algorithm is a combination of AdaGrad-Norm (my previous paper) and differential privacy. However, since the gradient is ``normalize"  by $b_t$, we must gain some "privacy" in this algorithm (better than Algorithm 1). Our research question for Algorithm 2 would be: \textbf{Can we improve privacy guarantee} and \textbf{what is the convergence rate and excess risk}? See Subsection 1.2.1 and 1.2.2 for the attempts to improve privacy guarantee and obtain an excess risk.
    
    \item[(2)] If we  can improve the  privacy  guarantee  for Algorithm 2, we might be able to extend  the  analysis to variants of SGD, such as normalized SGD  (the simplified version of \cite{cutkosky2020momentum}) that update as follows:
    $\theta_t=\theta_{t-1}-\eta n \frac{\nabla L(\theta_{t-1};z_{\xi_t})+c_t}{\|\nabla L(\theta_{t-1};z_{\xi_t})+c_t\|}$ with  $\xi_t\sim \text{Uniform}(1,...,n)$  and $c_t\sim \mathcal{N}(0,\sigma I).$
    
    % My conjecture would be  \emph{We could perhaps improve the privacy guarantee}.
 \item[(3)] Extend the analysis in the domain of federated learning with an emphasis on the data is non-i.i.d.
\end{itemize}

\textbf{Relevant work.} The most relevant work to the above question would be my work \cite{wu2019global,ward2019adagrad} and the recent NeurIPS20 \cite{zhou2020towards}. \cite{ward2019adagrad} gives a convergence guarantee $O(\sigma^2/\sqrt{T})$ for adaptive gradient methods but without Differential Privacy. \cite{zhou2020towards}  uses differential privacy theorem \cite{dwork2014algorithmic} to prove the generalization and convergence guarantee for the coordinate-wise adaptive gradient method.  However, the proof of the convergence can not distinguish adaptive stepsize from constant stepsize. %In other words, the takeaway from the paper is likely to be that you can prove generalization guarantee if DP framework is used. %Also,  convergence guarantee for adaptive gradient has been improved.  

Much recent work has been proposed to improve convergence, such as AdaClip (which adds less noise compared to the previous methods by using coordinate-wise adaptive clipping of the gradient) \cite{pichapati2019adaclip,chen2020understanding}. One can also improve privacy with different sampling method \cite{balle2020privacy}. For over-parameterized models, convergence rate has been improved by using method PDP-SGD \cite{zhou2021bypassing} where they leverage a low-dimensional structure of gradient space in deep networks. One can also connect the privacy algorithm with Langevin Dynamics \cite{wang2015privacy} and stochastic differential equations (SDE). There would be fruitful mathematical tools to analyze the convergence and privacy guarantees. 

==> olds/experiments.tex <==
\section{Experiments}



==> olds/intro.tex <==
\section{Introduction}
 Adaptive gradient methods such as AdaGrad \cite{duchi2011adaptive} or Adam \cite{kingma2014adam} are standard practice in modern machine learning community, particularly in large-scale natural language processing  \cite{vaswani2017attention,devlin2019bert,NEURIPS2020_1457c0d6,2020t5}. Empirical performances show that adaptive gradient methods are particularly beneficial to sparse gradient update \cite{duchi2011adaptive}.  Moreover, recents work provided both theoretical and empirical evidence that  the methods are highly adaptive to the noisy gradients, which results in less hyper-parameter tuning efforts on the learning rate \cite{levy2018online,ward2019adagrad,wu2019global}. 
 

 
Many researches have applied such methods in differential private learning and showed their empirical advantages over many other non-adaptive methods.   \cite{pmlr-v108-koskela20a} applied the learning rate adaptation to
DP-SGD and show its competitiveness to the well-tuned optimisation
methods.
\cite{9069364} developed a differentially private convolutional neural networks model with adaptive gradient descent methods by allocating each iteration’s privacy budget more carefully and obtain high prediction accuracy under modest privacy budget.
\cite{zhou2020towards} studied the generalization property of the private version of AdaGrad and performed deep learning tasks to show that private adaptive gradient methods and their variants outperform private SGD consistently.   \cite{bu2020deep} studied a private version of Adam (NoisyAdam) where they compared with private SGD (NoisySGD) and observed that the convergence of  NoisyAdam is much faster than NoisySGD in training tasks such as IMDB \cite{maas2011learning} and MovieLens 1M \cite{harper2015movielens} datasets.

However, given the successful empirical performance of adaptive gradient methods in differential private learning, the privacy analysis of such methods is limited.  It is often taken for granted that the privacy guarantees for adaptive gradient methods follows the same privacy guarantees as private SGD  \cite{zhou2020towards,bu2020deep}. However, we will show in this paper that this is not the case. 


The agenda:
\begin{itemize}
    \item Understand the theoretical guarantee for privacy guarantee of adaptive gradient methods such as AdaGrad-Norm, AdaGrad and RMSProp.
    \item Understand their optimization errors and excess risks. Try to get a tight bound of the optimization complexity/excess risk given the same privacy requirement. Tighten the dependence of the dimension -- possibly we could improve the dependence from $d$ to $\sqrt{d}$ or $\log(d)$.  For instance, current SGD is  $T=\mathcal{O}(n^2)$ to reach $O(\frac{1}{n})$ while maintain the $(\epsilon,\delta)$-DP where $\epsilon = \mathcal{O}(1)$. We need to improve $T$.
    \item Based on previous understanding, propose a better adaptive gradient methods that can have better optimization complexity while maintain comparable privacy guarantee.
    \item Numerical experiments in deep learning (privacy and accuracy)
\end{itemize}

% \subsection{Our Contribution.}
% \begin{itemize}
%     \item The theoretical  guarantee
% \end{itemize}

==> olds/privacy-guarantee-proof.tex <==

\begin{proof}

Without loss of generality, we assume $f(x)>0$ and let $f(x')=f(x)+1$. Since $\mathcal{M}(x) \sim \mathcal{N} \left(\frac{f(x)}{\sqrt{b^2+f(x)^2}}, \frac{\sigma_z^2}{b^2+f(x)^2} \right)$, we can get $\mathcal{L}_{\mathcal{M}}^{x,x'}(y)$  by applying Lemma \ref{lem:gaussian} with 
\begin{align}
 \sigma& = \frac{\sigma_z}{\sqrt{b^2+f(x)^2}}; \sigma'=  \frac{\sigma_z}{\sqrt{b^2+(f(x)+1)^2}} \text{ and } \rho = \sqrt{\frac{b^2+f(x)^2} {b^2+(f(x)+1)^2}}<1 \\
\mu &= \frac{f(x)}{\sqrt{b^2+f(x)^2}};  \mu' = \frac{(f(x)+1)}{\sqrt{b^2+(f(x)+1)^2}} \geq \mu.
\end{align}

\begin{lemma}
Let $Y\sim (\mu, \sigma)$ and $Y'\sim (\mu', \sigma')$.
With $\rho=\frac{\sigma'}{\sigma}$, we have then \begin{align}
    \ln\left(\frac{f_{X}(y)}{f_{X'}(y)}\right)
     &= \ln\left(\frac{\sigma'}{\sigma}\right) +\left(\frac{1}{2\sigma'^2}-\frac{1}{2\sigma^2} \right) y^2-\left(\frac{\mu'}{\sigma'^2}-\frac{\mu}{\sigma^2} \right)y+\left(\frac{\mu'^2}{2\sigma'^2}-\frac{\mu^2}{2\sigma^2}\right)\\
    &= \ln\left(\frac{\sigma'}{\sigma}\right) -\frac{\sigma'^{2}-\sigma^2}{2\sigma'^{2}\sigma^2} y^2-2y\frac{(\mu\sigma'^2-\mu'\sigma^2)}{2\sigma'^{2}\sigma^2} +\frac{(\mu^2\sigma'^2-\mu'^2\sigma^2)}{2\sigma'^{2}\sigma^2}\\
    &= \ln\left(\frac{\sigma'}{\sigma}\right) -\frac{\sigma'^{2}-\sigma^2}{2\sigma'^{2}\sigma^2}\left( y^2-2y\frac{\mu\sigma'^2-\mu'\sigma^2}{\sigma'^{2}-\sigma^2}+\frac{\mu^2\sigma'^2-\mu'^2\sigma^2 }{\sigma'^{2}-\sigma^2}\right)
\end{align}

\begin{align}
    \ln\left(\frac{f_{Y}(y)}{f_{Y'}(y)}\right) =  \frac{1}{2\sigma'^2}\left((1-\rho^2) y^2-2y(\mu'-\mu\rho^2)-(\mu^2\rho^2-\mu'^2)\right)+\ln\left(\rho\right). \label{eq:privacy-loss1}
\end{align} \label{lem:gaussian}
\end{lemma}

Thus we have 
\begin{align}
   \mathcal{L}_{\mathcal{M}}^{x,x'}(y) 
%   &= \ln\left(\rho\right) -\frac{\rho^2-1}{2\rho^2}\left( y^2-2y\frac{\mu\rho^2-\mu'}{\rho^2-1}+\frac{\mu^2\rho^2-\mu'^2 }{\rho^{2}-1}\right) \\
%     &= \ln\left(\rho\right) +\frac{1-\rho^2}{2\rho^2}\left( \left(y-\sqrt{\frac{\mu\rho^2-\mu'}{\rho^2-1}}\right)^2+\frac{\mu^2\rho^2-\mu'^2 +\mu'-\mu\rho^2}{\rho^{2}-1}\right) \\
&=\frac{1}{2\sigma'^2}\left((1-\rho^2) y^2-2y(\mu'-\mu\rho^2)\right)  -\frac{1}{2\sigma'^2}(\mu^2\rho^2-\mu'^2))+ \ln\left(\rho\right)\\
        % &= \frac{1-\rho^2}{2\rho^2} \left(y-\sqrt{\frac{\mu\rho^2-\mu'}{\rho^2-1}}\right)^2+\frac{\mu\rho^2(\mu-1)-\mu'(\mu' -1)}{2\rho^{2}}+  \ln\left(\rho\right)\\
 &= \left(y\sqrt{ \frac{1-\rho^2}{2\sigma'^2}}-\sqrt{\frac{\mu'-\mu\rho^2}{2\sigma'^2}}\right)^2-\frac{\mu\rho^2(\mu-1)-\mu'(\mu' -1)}{2\sigma'^2}+  \ln\left(\rho\right)\\
    &= \left(y\sqrt{ \frac{1-\rho^2}{2\sigma'^2}}-\sqrt{\frac{\mu'-\mu\rho^2}{2\sigma'^2}}\right)^2-\mathcal{T}_1+  \ln\left(\rho\right)
   \label{eq:privacy-loss2}
\end{align}
where we let \[\mathcal{T}_1 = \frac{\mu\rho^2(\mu-1)-\mu'(\mu' -1)}{2\sigma'^2}\]
% Plugging it back to \eqref{eq:privacy-def}, we simplify $Z_{\mathcal{M}}^{d,d'}$
% \begin{align}
% Z_{\mathcal{M}}^{d,d'}
% &=\log \left(\frac{v(d)}{v(d')} \exp \left(- \frac{(v(d)-a)^2- (v(d')-a)^2}{2\sigma^2}\right)\right)  \\
% &=- \frac{(v(d)-a)^2- (v(d')-a)^2}{2\sigma^2} + \log \left(\frac{v(d)}{v(d')}\right) 
% \end{align}

\paragraph{Compute $\mathbb{P}[L_{\mathcal{M}}^{x,x'}\geq \varepsilon]\leq \delta$}
\begin{lemma}
A mechanism $\mathcal{M}:\mathcal{X}\to \mathcal{Y}$ is $(\varepsilon, \delta)-DP$ if for any $x,x'\in \mathcal{X}$, we have 
$\mathbb{P}[L_{\mathcal{M}}^{x,x'}\geq \varepsilon]\leq \delta$.
\end{lemma}
Thus, we work on for any $\alpha>0$:
\begin{align}
\mathbb{P} \left(L_{\mathcal{M}}^{x,x'}\geq \varepsilon \right) &=\mathbb{P} \left(\exp\left(\alpha L_{\mathcal{M}}^{x,x'}\right) \geq \exp\left(\alpha\varepsilon\right) \right)
\leq \mathbb{E}\left[\exp\left(\alpha L_{\mathcal{M}}^{x,x'}\right)\right]/\exp(\alpha \varepsilon) 
%\\&= \mathbb{E}\left[\exp\left(\alpha Z_{\mathcal{M}}^{d,d'}(x)\right)\right]/\exp(\alpha \varepsilon)  \\
\end{align}
Using \eqref{eq:privacy-loss2}, we get
\begin{align}
 \mathbb{E}\left[\exp\left(\alpha L_{\mathcal{M}}^{x,x'}\right)\right]
 & =  \rho^{\alpha} \exp\left(\alpha\mathcal{T}_1\right)\mathbb{E}_{\mathcal{M}(x)}\left[\exp\left( \underbrace{\mathcal{M}(x)\sqrt{ \frac{ \alpha (1-\rho^2)}{2\sigma'^2}}-\sqrt{\frac{\alpha (\mu'-\mu\rho^2)}{2\sigma'^2}}}_{X_{\mathcal{M},\rho,\mu,\mu'} }\right)^2\right] \\
 & =  \frac{\rho^{\alpha} \exp\left(-\alpha\mathcal{T}_1\right)}{\sqrt{1-   \alpha\sigma_z^2(1-\rho^2) \rho^2}}\exp\left(\frac{1}{1- \alpha\sigma_z^2(1-\rho^2) \rho^2} \left(\mu\sqrt{ \frac{\alpha (1-\rho^2)}{2\sigma'^2}} -\sqrt{\frac{\alpha (\mu'-\mu\rho^2)}{2\sigma'^2}}  \right)^2\right)
\end{align}
where the last equality Lemma \ref{lem:square-gaussian} is applied to Gaussian $X_{\mathcal{M},\rho,\mu,\mu'} =(\mu +\sigma Z)\sqrt{ \frac{\alpha (1-\rho^2)}{2\sigma'^2}}-\sqrt{\frac{\alpha (\mu'-\mu\rho^2)}{2\sigma'^2}}$  with
\begin{align}
    \mathbb{E}\left[X_{\mathcal{M},\rho,\mu,\mu'} \right]=\mu\sqrt{ \frac{\alpha (1-\rho^2)}{2\sigma'^2}} -\sqrt{\frac{\alpha (\mu'-\mu\rho^2)}{2\sigma'^2}} \text{ and } \text{Var}\left[X_{\mathcal{M},\rho,\mu,\mu'} \right]= \frac{\alpha \sigma^2\sigma_z^2(1-\rho^2)}{2\sigma'^2} =\frac{1}{2} \alpha\sigma_z^2(1-\rho^2) \rho^2
\end{align}
\begin{lemma}
Let $Y \sim \mathcal{N} (\mu, \sigma)$ with $\sigma^2\leq \frac{1}{2}$, we have  $\mathbb{E}[\exp(Y^2)]=\frac{1}{\sqrt{1-2\sigma^2}}\exp(\frac{\mu^2}{1-2\sigma^2})$. \label{lem:square-gaussian}
\end{lemma}


Let us continue the analysis of privacy by making a further simplification: let us assume $f(x) = 0$ which implies the following

\begin{align*}
    \mu &= 0, \\
    \sigma &= \frac{\sigma_z}{b}\\
    \mu' &= \frac{1}{\sqrt{b^2+1}} \\
    \sigma' &= \frac{\sigma_z}{\sqrt{b^2+1}} \\
    \mathcal{T}_1 &= \frac{- \mu'(\mu' -1)}{2  \sigma'^2} =  \frac{ \mu'(1-\mu')}{2 \sigma'^2}\\
    \rho &= \sqrt{\frac{b^2}{b^2+1}}
\end{align*}

\noindent By plugging in $\rho$ in the expression of $\mathcal{T}_1$ we have that
\begin{align*}
    \mathcal{T}_1 = \frac{\sqrt{b^2 +1}}{2\sigma_z^2}(1 - \frac{1}{\sqrt{b^2+1}})%\frac{b^2 +1}{\sqrt{b^2+1}(b^2 - \alpha\frac{\sigma_z^4}{b^2 +1})} \\
    = \frac{\sqrt{b^2+1} -1}{2\sigma_z^2} 
    = \frac{b^2}{2\sigma_z^2(1+\sqrt{b^2+1})} 
    %\leq  \frac{1}{\sqrt{b^2+1}}.
\end{align*}

% \［\mathcal{T}_1 = \frac{- \mu'(\mu' -1)}{2 \rho^2} = \frac{\sqrt{b^2+1}}{2b^2}(1 - \frac{1}{\sqrt{b^2+1}})= \frac{\sqrt{b^2 +1}}{2b^2}(1 - \frac{1}{\sqrt{b^2+1}})
%     = \frac{\sqrt{b^2+1} -1}{2b^2} 
%     = \frac{b^2}{2b^2(1+\sqrt{b^2+1})} 
%     = \frac{1}{2(\sqrt{b^2+1}+1)}.\］

\noindent By plugging in the expression of $\rho$ and setting the number under the square root $\sqrt{1 - \frac{\alpha \sigma^2 \sigma_z^2(1- \rho^2)}{\sigma'^2}}$ to be greater than or equal to zero, we obtain the following constraint on $\alpha$

\begin{align}
    \alpha \leq \frac{1}{\sigma_z^2\rho^2(1-\rho^2)}=\left(\frac{b^2+1}{b^2\sigma_z}\right)^2.
\end{align}
% \me{starting here}
% \noindent Now, let us go back to further computing $\mathbb{E}(\exp(\alpha \mathcal{L}_{M}^{x, x'}))$:

% \begin{align}
% \mathbb{E}\left[\exp(\alpha \mathcal{L}_{M}^{x, x'})\right]&= \frac{\rho^2 \rho \exp(-\alpha \mathcal{T}_1)}{\sqrt{\frac{1}{b^2+1} (b^2 - \alpha\frac{\sigma_z^4}{b^2+1})}} 
% \exp \left( \frac{\rho^2}{\frac{1}{b^2+1}(b^2 - \alpha \frac{\sigma_z^4}{b^2 +1})}\cdot \frac{\alpha \mu'}{2\rho^2} \right)\\
% &=\frac{\rho^{\alpha +1}}{\sqrt{\frac{1}{b^2+1} (b^2 - \alpha\frac{\sigma_z^4}{b^2+1})}} \exp \left( \frac{\alpha\sqrt{b^2+1}}{(b^2 - \alpha \frac{\sigma_z^4}{b^2 +1})} -\frac{\alpha}{2(\sqrt{b^2+1}+1)} \right)\\
% &\leq  \exp \left( \frac{\alpha\sqrt{b^2+1}}{(b^2 - \alpha \frac{\sigma_z^4}{b^2 +1})} -\frac{\alpha}{2(\sqrt{b^2+1}+1)} \right) 
% % \\
% % &=  \exp \left( \frac{\alpha (b^2+1) +\alpha(b^2 - \alpha \frac{\sigma_z^4}{b^2 +1})  }{b^2\sqrt{b^2+1} - \alpha \frac{\sigma_z^4}{\sqrt{b^2+1}}} \right)
% \end{align}
% where the inequality is due to our chosen $\alpha$ such that 
% \begin{align}
%     \frac{\rho^{\alpha +1}}{\sqrt{\frac{1}{b^2+1} (b^2 - \alpha\frac{\sigma_z^4}{b^2+1})}} \leq 1
% \end{align}
% \noindent We now need 
% \begin{align}
%      &\exp \left( \frac{\alpha\sqrt{b^2+1}}{(b^2 - \alpha \frac{\sigma_z^4}{b^2 +1})} -\frac{\alpha}{2(\sqrt{b^2+1}+1)} -\varepsilon \alpha\right) \leq \delta \\
%      \Leftrightarrow  \quad &   -\frac{\alpha\sqrt{b^2+1}}{(b^2 - \alpha \frac{\sigma_z^4}{b^2 +1})} +\alpha\left(\frac{1}{2(\sqrt{b^2+1}+1)} +\varepsilon \right) \geq \ln \left( \frac{1}{\delta}\right) 
% \end{align}
% Thus the above is satisfied if we have following
% \begin{align}
% & \alpha\left(\frac{1}{2(\sqrt{b^2+1}+1)} +\varepsilon \right) = 2\ln \left( \frac{1}{\delta}\right)  \label{eq:first} \\
%  &-\frac{\alpha\sqrt{b^2+1}}{(b^2 - \alpha \frac{\sigma_z^4}{b^2 +1})} \geq -\ln \left( \frac{1}{\delta}\right) \label{eq:second}
% \end{align}
% Note that  \eqref{eq:second} gives
% \begin{align}
% \frac{1}{\alpha}\geq \frac{\sqrt{b^2+1}}{b^2\ln(1/\delta)}+\frac{\sigma_z^4}{b^2(b^2+1)}
% \end{align}
% and  thus using \eqref{eq:first} gives
% \begin{align}
% \varepsilon+\frac{1}{2(\sqrt{b^2+1}+1)}  =\frac{2\ln(1/\delta)}{\alpha}\geq \frac{2\sqrt{b^2+1}}{b^2}+\frac{2\sigma_z^4\ln(1/\delta)}{b^2(b^2+1)}
% \end{align}
% \me{This implies that large $b$ give small $\varepsilon$ and so higher privacy. However, when the term $\frac{2\sigma_z^4\ln(1/\delta)}{b^2(b^2+1)}$ implies large $\sigma_z$ gives large $\varepsilon$ and so low privacy, which seems not reasonable.}

% \medksip


\irina{Beginning redo-ing the computations from equation 16 above, after correcting for a mistake}

We start by writing out $ \mathbb{E}[\exp(\alpha \mathcal{L}_{M}^{x, x'})]$ and plugging in $\mu = 0$, then plugging in for $\mathcal{T}_1$, and $\rho$, we get that:

\begin{align}
    \mathbb{E}[\exp(\alpha \mathcal{L}_{M}^{x, x'})] &= \frac{\rho^{\alpha}\exp(-\alpha \mathcal{T}_1)}{\sqrt{1 -\alpha \sigma_z^2 (1-\rho^2)\rho^2}}\cdot \exp \left( \frac{1}{1 -  \alpha \sigma_z^2 (1-\rho^2)\rho^2} \left(\mu \sqrt{\frac{\alpha(1-\rho^2)}{2\sigma'^2}} - \sqrt{\frac{\alpha(\mu' - \mu\rho^2)}{2\sigma'^2}}\right)^2\right) \\
    &= \frac{\rho^{\alpha} \exp{(-\alpha \mathcal{T}_1})}{\sqrt{1 - \alpha \sigma_z^2(1-\rho^2) \rho^2}} \cdot \exp \left( \frac{1}{1 -\alpha \sigma_z^2 (1-\rho^2) \rho^2} \cdot \frac{\alpha \mu'}{2\sigma'^2}\right) \\
    &=\frac{\rho^{\alpha} e^{-\frac{\alpha b^2}{2\sigma_z^2(1+  \sqrt{b^2 +1})}}}{\sqrt{1 - \alpha \sigma_z^2\frac{b^2}{(b^2 +1)^2}}} \exp \left( \frac{1}{1 - \frac{\alpha \sigma_z^2 b^2}{(b^2 +1)^2}} \cdot \frac{\alpha \sqrt{b^2+1}}{2\sigma_z^2}\right) \\
    &= \frac{\rho^{\alpha}}{\sqrt{1 -  \alpha \sigma_z^2 \frac{b^2}{(b^2+1)^2}}} \cdot \exp \left( \frac{2 \alpha (b^2 +1)^{2.5} }{(2(b^2 +1)^2 - \alpha\sigma_z^2 b^2)\cdot 2\sigma_z^2 } - \frac{\alpha b^2}{2\sigma_z^2(1 + \sqrt{1 +b^2})}\right)\\
    &\leq \exp\left( \frac{(b^2+1)^{2.5}\alpha/ \sigma_z^2}{(2(b^2 +1)^2 - \alpha \sigma_z^2 b^2) } - \frac{\alpha b^2}{2 \sigma_z^2(1+ \sqrt{1+b^2})}\right).
\end{align}

\noindent In order to have $(\varepsilon, \delta)$-differential privacy, we need to choose $\alpha $ appropriately so that the following is satisfied

\begin{align}
    \exp \left (\frac{(b^2 +1)^{2.5} \alpha/\sigma_z^2}{2(b^2+1)^2 - \alpha \sigma_z^2 b^2} - \frac{\alpha b^2}{2\sigma_z^2(1+ \sqrt{1+ b^2})} - \varepsilon \alpha\right) &\leq \delta \\
   - \frac{(b^2+1)^{2.5}\alpha/ \sigma_z^2}{(2(b^2+1)^2 - \alpha \sigma_z^2 b^2)} + \alpha \left( \frac{b^2}{2\sigma_z^2(1 + \sqrt{1 + b^2} )} + \varepsilon \right) &\geq \ln(\frac{1}{\delta}). 
\end{align}

\noindent The above is satisfied if


\begin{align}
    \alpha\left(\frac{b^2}{2\sigma_z^2(1 + \sqrt{1 + b^2})}+ \varepsilon  \right) &= 2 \ln(\frac{1}{\delta}) \\
    -\frac{ (b^2 +1)^{2.5}\alpha/ \sigma_z^2}{2(b^2+1)^2 - \alpha \sigma_z^2 b^2} &\geq - \ln(\frac{1}{\delta}). 
\end{align}

From equation (34)  we have that

\begin{align}
    \frac{1}{\alpha} \geq \frac{\sqrt{b^2+1}}{2\sigma_z^2\ln(1/\delta)} + \frac{\sigma_z^2b^2}{2(b^2+1)^2}
\end{align}

By using  the above in equation (33), we obtain that

\begin{align}
    \varepsilon &\geq -\frac{b^2}{2\sigma_z^2(1 + \sqrt{1 + b^2})}+ \frac{\sqrt{b^2 +1}}{\sigma_z^2} + \ln \left(\frac{1}{\delta} \right) \left(\frac{\sigma_zb}{b^2 +1}\right)^2 \\
    &= \frac{2\sqrt{b^2 +1}(1+\sqrt{b^2 +1}) -b^2}{2\sigma_z^2(1 + \sqrt{1 + b^2})} + \ln \left(\frac{1}{\delta} \right) \left(\frac{\sigma_zb}{b^2 +1}\right)^2 \\
        &= \frac{1}{\sigma_z^2} \left(1+\frac{b^2}{2(1 + \sqrt{1 + b^2})}\right) + \ln \left(\frac{1}{\delta} \right) \left(\frac{b}{b^2 +1}\right)^2 \sigma_z^2
        % \\
        % &= \mathcal{O}\frac{1}{\sigma_z^2} \left(1+\frac{b^2}{2(1 + \sqrt{1 + b^2})}\right) + \ln \left(\frac{1}{\delta} \right) \left(\frac{b}{b^2 +1}\right)^2 \sigma_z^2 \\
        % \\
        % &\geq \left(\frac{b}{b^2 +1}\right)\sqrt{\ln \left(\frac{1}{\delta} \right) \left(1+\frac{b^2}{2(1 + \sqrt{1 + b^2})}\right)}   \\        
\end{align}




\end{proof}


\irina{Attempt to  generalize the computation for $f(x) \neq 0$. }


Let us assume, in this more general case, that $f(x) = x$ and $f(x') = x+1$. This way, we obtain the following

\begin{align*}
    \mu &= \frac{x}{\sqrt{b^2 + x^2} } \\
    \mu' &= \frac{x+1}{\sqrt{b^2 + (x+1)^2}} \\
    \sigma &= \frac{\sigma_z}{\sqrt{b^2+x^2}} \\
    \sigma' &= \frac{\sigma_z}{\sqrt{b^2 + (x+1)^2}} \\
    \rho &= \frac{\sigma'}{\sigma} = \frac{\sqrt{b^2 +x^2}}{\sqrt{b^2 + (x+1)^2}} \\
    \mathcal{T}_1 &= \frac{\mu \rho^2 (\mu -1) - \mu'(\mu'-1)}{2\sigma'^2} = \frac{(x+1)(\sqrt{b^2 +(x+1)^2} -1) -x(\sqrt{b^2+x^2}+1)}{2\sigma_z^2} \\
    & \geq \frac{1}{2\sigma_z^2}[(x+1)(\sqrt{b^2+x^2} -1) -x(\sqrt{b^2 +x^2} +1)] = \frac{1}{2\sigma_z^2}(\sqrt{b^2 +x^2}-2x-1). \\
\end{align*}

\noindent We now want to examine the following function

\begin{align*}
    h(x) &= \mathbb{E}[\exp(\alpha \mathcal{L}_M^{x, x'})] \\ 
    &= \frac{\rho^{\alpha}\exp(-\alpha \mathcal{T}_1)}{\sqrt{1 - \alpha \sigma_z^2(1-\rho^2)\rho^2}}\exp\left(\frac{1}{1-\alpha \sigma_z^2 (1-\rho^2)\rho^2}  \cdot \left( \mu \sqrt{\frac{\alpha(1-\rho^2)}{2\sigma'^2}} -\sqrt{\frac{\alpha(\mu' - \mu \rho^2)}{2\sigma'^2}} \right)^2\right)
 \end{align*}

\noindent Let us examine the terms appearing in the expression of $h(x)$ one by one, possibly simplifying them by means of upper bounds. 

\noindent First of all, we have that

\begin{align*}
    \rho^{\alpha}\exp(-\alpha \mathcal{T}_1) &\leq 1\cdot \exp(-\alpha\mathcal{T}_1)  \\
    & \leq \exp \left( - \frac{\alpha}{2\sigma_z^2}(\sqrt{b^2 +x^2}-2x-1)\right). 
\end{align*}

\noindent Next, we look at the term $\frac{1}{\sqrt{1 - \alpha \sigma_z^2(1-\rho^2)\rho^2}}$:

\begin{align*}
    \frac{1}{\sqrt{1 - \alpha \sigma_z^2(1-\rho^2)\rho^2}} &= \frac{1}{\sqrt{1- \alpha \sigma_z^2 \frac{(2x+1)(b^2 +x^2)}{(b^2+(x+1)^2)^2}}} \\
    & \leq  \frac{1}{\sqrt{1- \alpha \sigma_z^2 \frac{(2x+1)(b^2 +x^2)}{(b^2+x^2)^2}}} \\
    &= \frac{1}{\sqrt{1- \alpha \sigma_z^2 \frac{2x+1}{b^2 + x^2}}}. 
\end{align*}


\noindent Let us now look at the term $\left( \mu \sqrt{\frac{\alpha(1-\rho^2)}{2\sigma'^2}} -\sqrt{\frac{\alpha(\mu' - \mu \rho^2)}{2\sigma'^2}} \right)^2$:

\begin{align*}
    \left( \mu \sqrt{\frac{\alpha(1-\rho^2)}{2\sigma'^2}} -\sqrt{\frac{\alpha(\mu' - \mu \rho^2)}{2\sigma'^2}} \right)^2 &= \left( \frac{x\sqrt{\alpha(2x+1)}}{\sqrt{b^2 + x^2}\sqrt{2} \sigma_z} - \frac{\sqrt{\alpha(\sqrt{b^2 +(x+1)^2}(x+1) -x\sqrt{b^2 + x^2})}}{\sqrt{2}\sigma_z} \right)^2 \\
    &\leq 2 \frac{x^2 \alpha (2x+1)}{2\sigma_z^2(b^2 + x^2)} + 2 \frac{\alpha(\sqrt{b^2 + (x+1^2)}(x+1) - x\sqrt{b^2 + x^2})}{2 \sigma_z^2} \\
    & \leq \frac{\alpha x^2 (2x+1)}{\sigma_z^2 (b^2 + x^2)} + \frac{\alpha \sqrt{b^2 + (x+1)^2}}{\sigma_z^2} \\
    & \leq \frac{\alpha(x^2(2x+1) + (b^2 + x^2)\sqrt{b^2 + (x+1)^2})}{\sigma_z^2(b^2 + x^2)}
\end{align*}

\noindent By combining all of the above bounds, we can re-analyze the expression of $h(x)$ and obtain the following

\begin{align*}
    h(x) &\leq \frac{1}{\sqrt{1 - \alpha \sigma_z^2\frac{2x+1}{b^2+x^2}}} \cdot \exp \left( \frac{1}{1- \alpha \sigma_z^2 \frac{2x+1}{b^2 + x^2}} \cdot 
    \frac{\alpha}{\sigma_z^2} \frac{x^2(2x+1)+(b^2 + x^2)\sqrt{b^2 + (x+1)^2}}{b^2 + x^2}
    - \frac{\alpha}{2\sigma_z^2}(\sqrt{b^2 +x^2} - (2x+1)) \right)
\end{align*}




==> olds/privacy-guarantee.tex <==
\section{Some general approach to think about privacy and convergence}
Let us think about the general update
\begin{minipage}[t]{0.5\textwidth}
\begin{algorithm}[H]
\caption{\textbf{Private SGD} (version 2)}
\label{alg:privacy-general}
\begin{algorithmic}[1]
	    \State Input $\theta_0,b_t$,
	    \For {$ t=1,\ldots,T$} 
	      \State $\xi_t\sim \text{Uniform}(1,...,n)$  and $c_t\sim \mathcal{N}(0,\sigma I)$
	    \State update $b_{t+1}$	 and $b'_{t+1}$ with certain rule    
	   % \State $G_{t}= ,$ where
	    \State update $\theta_{t+1}=\theta_{t}-  \frac{\eta}{b_{t+1}}(\nabla L(\theta_{t};x_{\xi_t})+b'_{t+1}c_t)$
	    \EndFor
\end{algorithmic}
\end{algorithm}
\end{minipage}

\begin{prop}
Let $Z\sim\mathcal{N}(0,\sigma_z^2)$. At iteration $t$ in Algorithm \ref{alg:privacy-general}, we have the privacy mechanism $\mathcal{M}_t:\mathbb{R}^d\to\mathbb{R}^d$ for $f_t(X)=\nabla L(\theta_t;x_{\xi_t})$  with $x_{\xi_t}\sim X$ :
%some $f(X):\mathbb{R}\to\mathbb{R}$ and $b(X):\mathbb{R}\to\mathbb{R}$ follows
\[\mathcal{M}^{\text{SGD}}_t(X)=f_t(X)+ b'_{t+1}Z.\]
\end{prop}
The above proposition is easily verified by checking the line 5 in Algorithm \ref{alg:privacy-general}.  It is easy to get from Lemma \ref{lem:gaussian} that each step for a fixed $\sigma_z$ we have $(\epsilon_t, \delta)$-DP where 
\[\varepsilon_t = \frac{ \sqrt{2G\ln(1.25/\delta)}}{ n\sigma_zb'_{t+1}}\]
 Using  extended advanced composition \ref{thm:advanced-comp}, we have the final output follow $(\varepsilon_{gen}, \delta_{\text{gen}})-DP$ where 
 \begin{align}
   \varepsilon_{com}(t) &= \sqrt{\sum_{i=0}^{t-1} \varepsilon_i^2 \log\left(\frac{1}{\delta}\right)} +  \sum_{i=0}^{t-1} \frac{\varepsilon_i^2}{2+\varepsilon_i} \\
   &\leq 2G\sqrt{\sum_{t=0}^{T-1} \varepsilon_t^2 \log\left(\frac{1}{\delta'}\right)}\\
   &= \frac{2\sqrt{2\log\left({1}/{\delta'}\right)\log\left({1.25}/{\delta_0}\right)}}{n  \sigma_z} \sqrt{\sum_{t=1}^{T-1}  \frac{ 1}{b'^2_{t+1}}  }      
\end{align}
Here, in the first inequality, the term $\sum_{i=1}^K \frac{\varepsilon_t^2}{2+\varepsilon_t}$ is considerable smaller  than $\sqrt{\sum_{t=0}^{T-1} \varepsilon_t^2 \log\left(\frac{1}{\delta_0}\right)}$. Thus, 
 \begin{align}
    \sigma_z
   &= \frac{2G\sqrt{2\log\left({1}/{\delta'}\right)\log\left({1.25}/{\delta_0}\right)}}{n \varepsilon_{gen} } \sqrt{\sum_{t=1}^{T-1}  \frac{ 1}{b'^2_{t+1}}  }      
\end{align}

%  \begin{align}
%   b_\tau = (a+c\tau)^p
% \end{align}
%  \begin{align}
%     \varepsilon_{gen}
%   &= \frac{2G\log\left({1}/{\delta}\right)}{n \sigma_z } \sqrt{\sum_{\tau=1}^{t-1}  \frac{ 1}{b^2_{\tau+1}}  }      
% \end{align}


\subsection{Convergence}
Assume
\begin{enumerate}
\item[A1] The random vectors $\xi_k$, $k = 0,1,2, \dots, $ are independent of each other and also of $x_k$;
% \item[A2] $\mathbb{E}_{\xi_k}[ \| G(x_k, \xi_k) -\nabla F(x_k) \|^2] \leq \sigma_G^2;$
\item[A2] $\| \nabla F(x) \|^2 \leq G^2$ uniformly.
\end{enumerate}
Recall the update in Algorithm \ref{alg:privacy-general}:
\begin{align*}
\theta_{t+1}&= \theta_t -  \frac{\eta }{b_{t+1}}G_t - \eta\frac{b'_{t+1}}{b_{t+1}} Z \text{  with } G_t=\nabla L(\theta_{t};x_{\xi_t})
\end{align*}
By Lipschitz gradient smoothness:
\begin{align}
L(\theta_{j+1}) &\leq L(\theta_{j}) - \eta\langle{ \nabla L(\theta_j),\frac{1 }{b_{j+1}}G_j - \frac{b'_{j+1}}{b_{j+1}} Z\rangle}+\frac{ \eta^2 L}{2} \left\| \frac{ G_j}{b_{j+1}}+ \frac{b'_{j+1}}{b_{j+1}} z_j  \right\|^2 \nonumber \\
\mathbb{E}[L(\theta_{j+1})] &\leq \mathbb{E}[L(\theta_{j})] -\frac{ \eta \mathbb{E}[\|\nabla L(\theta_{j})\|^2]}{b_{j+1}} +\frac{ \eta ^2 L}{2b_{j+1}^2} \mathbb{E}[\|G_j\|^2]  + \frac{ \eta ^2 d L \sigma_z^2}{2}\frac{b'^2_{j+1}}{b_{j+1}^2} % \label{remark2}
\end{align}

So we have%think about $\eta_t = \frac{\eta}{\sqrt{b^2_{0}+ tc_b}}$
\begin{align}
\sum_{\ell=0}^{T-1}\frac{ 1}{b_{\ell+1}} \sum_{\ell=0}^{T-1} \frac{b_{\ell+1}}{\sum_{\ell=0}^{T-1} \frac{ 1}{b_{\ell+1}}}\mathbb{E} \|\nabla L(\theta_\ell)\|^2
   & \leq \sum_{\ell=0}^{T-1}\frac{\mathbb{E}  \|\nabla L(\theta_\ell)\|^2}{b_{\ell+1}} \\
   & \leq  \frac{\mathbb{E}[L(\theta_{0})]  }{\eta}+ \frac{\eta L}{2}\sum_{\ell=0}^{T-1} \frac{ \mathbb{E}[\|G_\ell\|^2]}{b^2_{\ell+1}}  + \frac{ \eta d L \sigma_z^2}{2}\sum_{\ell=0}^{T-1} \left(\frac{b'_{\ell+1}}{b_{\ell+1}} \right)^2 \\
   \Rightarrow  \sum_{\ell=0}^{T-1}\frac{ 1}{b_{\ell+1}}\sum_{\ell=0}^{T-1}  w_{\ell}\mathbb{E} \|\nabla L(\theta_\ell)\|^2
   & \leq  \frac{\mathbb{E}[L(\theta_{0})]}{\eta} + \frac{\eta L}{2}\sum_{\ell=0}^{T-1} \frac{ \mathbb{E}[\|G_\ell\|^2]}{b^2_{\ell+1}} + \frac{ \eta d LG^2 \log^2(1/\delta) }{2n^2\varepsilon^2_{gen} }\sum_{\ell=0}^{T-1} \frac{ b'^2_{\ell+1}}{b^2_{\ell+1}}  \sum_{\ell=1}^{T-1}  \frac{ 1}{b'^2_{\ell+1}} \nonumber  \\ 
      & \leq  B_1 + \frac{B_2}{n^2}  \label{eq:bound-general}
\end{align}
where we let $B_1  =   \frac{\mathbb{E}[L(\theta_{0})]}{\eta} + \frac{\eta L}{2}\sum_{\ell=0}^{T-1} \frac{ \mathbb{E}[\|G_\ell\|^2]}{b^2_{\ell+1}}$ and $B_2= \frac{ \eta d LG^2 \log^2(1/\delta) }{2\varepsilon^2_{gen} }\sum_{\ell=0}^{T-1} \frac{ b'^2_{\ell+1}}{b^2_{\ell+1}}\sum_{\ell=1}^{T-1}  \frac{ 1}{b'^2_{\ell+1}}   $.

The optimal bound for the the right  hand side of  above inequality is when $B_1=\frac{B_2}{n^2}$  and so
\begin{align}
\sum_{\ell=0}^{T-1}\frac{ 1}{b_{\ell+1}}\sum_{\ell=0}^{T-1}  w_{\ell}\mathbb{E} \|\nabla L(\theta_\ell)\|^2\leq \frac{\sqrt{2B_1B_2}}{n}
\end{align}

Thus, the convergence is
     \begin{align}
      \sum_{\ell=0}^{T-1}  w_{\ell}\mathbb{E} \|\nabla L(\theta_\ell)\|^2 \leq\frac{1}{n} \frac{\sqrt{2B_1B_2}}{  \sum_{\ell=0}^{T-1}\frac{ 1}{b_{\ell+1}}  }  \label{eq:bound-b1b2}   % \sqrt{2\left( \mathbb{E}[L(\theta_{0})] + \frac{\eta L}{2}\sum_{\ell=0}^{T-1} \frac{ \mathbb{E}[\|G_\ell\|^2]}{b^2_{\ell+1}}\right)\left( \frac{\eta^2 d LG^2 \log^2(1/\delta) }{2n^2\varepsilon^2_{gen}}\sum_{\ell=0}^{T-1} \frac{ b'^2_{\ell+1}}{b^2_{\ell+1}}  \sum_{\ell=1}^{T-1}  \frac{ 1}{b'^2_{\ell+1}}             \right)   }
     \end{align}
Note that  $B_1=\frac{B_2}{n^2}$  implies
\begin{align}
\quad & n^2  =  \frac{B_2}{B_1}=\frac{  \frac{\eta^2 d LG^2 \log^2(1/\delta) }{2n^2\varepsilon^2_{gen}}\sum_{\ell=0}^{T-1} \frac{ b'^2_{\ell+1}}{b^2_{\ell+1}}  \sum_{\ell=1}^{T-1}  \frac{ 1}{b'^2_{\ell+1}}             }{ \mathbb{E}[L(\theta_{0})] + \frac{\eta^2 L}{2}\sum_{\ell=0}^{T-1} \frac{ \mathbb{E}[\|G_\ell\|^2]}{b^2_{\ell+1}} }
\end{align}
Now the question is 
\begin{center}
What is the optimal relationship between $b'_{t}$ and ${b_t}$ such that  the bound $B_2$ is tight. \\
Can we optimize the  complexity $T$ in terms of $n$ with larger stepsize ${1/b_t}$
\end{center}

\subsection{Optimal relationship between $b'_{t}$ and ${b_t}$ for tight $B_2$ }
Note that $b'_{t}$ affect only $B_2$. Note  that 
\begin{align}
  \sum_{\ell=0}^{T-1} \frac{ b'^2_{\ell+1}}{b^2_{\ell+1}}  \sum_{\ell=1}^{T-1}  \frac{ 1}{b'^2_{\ell+1}}      \geq   \left(\sum_{\ell=0}^{T-1}\sqrt{ \frac{ b'^2_{\ell+1}}{b^2_{\ell+1}} }\sqrt{   \frac{ 1}{b'^2_{\ell+1}}}  \right)^2  =\left( \sum_{\ell=0}^{T-1} \frac{ 1}{b_{\ell+1}}  \right)^2
\end{align}
where we apply the fact that  $|\langle{w,v\rangle}|^2\leq \|w\|^2\|v\|^2 $ and the equality holds  when $ \frac{ b'_{\ell+1}}{b_{\ell+1}}    =  \frac{ 1}{b'_{\ell+1}}   $.  So the optimal relationship is
\begin{align}
 b'^2_{\ell}=b_{\ell}.   
\end{align}
Thus  $B_2$ reduces to 
\begin{align}
    B_2 = \frac{ \eta d LG^2 \log^2(1/\delta) }{2\varepsilon^2_{gen} } \left( \sum_{\ell=0}^{T-1} \frac{ 1}{b_{\ell+1}}  \right)^2
\end{align}
and 
\begin{align}
 n^2  =  \frac{B_2}{B_1}=\frac{  \frac{\eta^2 d LG^2 \log^2(1/\delta) }{2\varepsilon^2_{gen}}     \left( \sum_{\ell=0}^{T-1} \frac{ 1}{b_{\ell+1}}  \right)^2       }{ \mathbb{E}[L(\theta_{0})] + \frac{\eta^2 L}{2}\sum_{\ell=0}^{T-1} \frac{ \mathbb{E}[\|G_\ell\|^2]}{b^2_{\ell+1}} } 
 \leq \frac{ d G^2 \log^2(1/\delta)     \left( \sum_{\ell=0}^{T-1} \frac{ 1}{b_{\ell+1}}  \right)^2       }{\varepsilon^2_{gen}\sum_{\ell=0}^{T-1} \frac{ \mathbb{E}[\|G_\ell\|^2]}{b^2_{\ell+1}} }\label{eq:n-square}
\end{align}
Thus the inequality \ref{eq:bound-b1b2} becomes
\begin{align}
\sum_{\ell=0}^{T-1}  w_{\ell}\mathbb{E} \|\nabla L(\theta_\ell)\|^2 &\leq \frac{\sqrt{2B_1B_2}}{n\sum_{\ell=0}^{T-1}\frac{ 1}{b_{\ell+1}}} \\
  &\leq \frac{\sqrt{B_1}}{n} \frac{\sqrt{\eta d L} G \log (1/\delta) }{\varepsilon_{gen} } 
  \\
%   &\leq \frac{1}{n} \frac{\sqrt{B_1\eta dL} G \log (1/\delta) }{\varepsilon_{gen} }
%   \\
      &= \frac{1}{n} \frac{\sqrt{\eta dL} G \log (1/\delta) }{\varepsilon_{gen} }    \sqrt{\frac{\mathbb{E}[L(\theta_{0})]}{\eta} + \frac{\eta L}{2}\sum_{\ell=0}^{T-1} \frac{ \mathbb{E}[\|G_\ell\|^2]}{b^2_{\ell+1}} } \label{eq:bound-optimal}
%\\
\end{align}

    

% To get  a tight bound  in $B_2$,
  

\subsection{Convergence bound with optimal relationship $b'^2_t=b_t$}
Suppose  $b_{t}={(a+ct)^p}$ with $p>0$ and then we have 
\begin{align}
\sum_{\ell=0}^{T-1} \frac{ 1}{(1+t)^{p}}\leq  1+
\begin{cases} 
 \frac{1}{1-p}T^{1-p} & p<1\\
\log(1+T) & p=1\\
%   \frac{1}{p-1}\left(1-T^{1-p}\right)& p>1
    \frac{1}{p-1}& p>1
\end{cases}
\end{align}
\begin{align}
\sum_{\ell=0}^{T-1} \frac{ 1}{(1+t)^{p}}\geq  
\begin{cases} 
 \frac{1}{1-p}\left(T^{1-p}-1\right) & p<1\\
\log(1+T)-1 & p=1\\
%   \frac{1}{p-1}\left(1-T^{1-p}\right)& p>1
   1& p>1
\end{cases}
\end{align}
% \quad\text{and} \quad \sum_{\ell=0}^{T-1} \frac{ 1}{(1+t)^{2p}}\leq 
% \begin{cases} \log(1+T) & p=0.5\\
% T^{1-2p} & \text{else}
% \end{cases}

\begin{align}
    B_1 = \frac{\mathbb{E}[L(\theta_{0})]}{\eta} + \frac{\eta L}{2}\sum_{\ell=0}^{T-1} \frac{ \mathbb{E}[\|G_\ell\|^2]}{b^2_{\ell+1}}
    &\leq   \frac{\mathbb{E}[L(\theta_{0})]}{\eta} + \frac{\eta L}{2}G^2\sum_{\ell=0}^{T-1} \frac{ 1}{(1+t)^{2p}}\\
   &\leq  \frac{\mathbb{E}[L(\theta_{0})]}{\eta} + 
   \begin{cases} 
   \frac{\eta L}{2(1-2p)}G^2T^{1-2p} & p<0.5\\
\frac{\eta L}{2}G^2\log(1+T) & p=0.5\\
\frac{\eta L}{2(2p-1)}G^2& p>0.5
\end{cases}
\end{align}
\begin{align}
    B_2 = \frac{ \eta d LG^2 \log^2(1/\delta) }{2\varepsilon^2_{gen} } \left( \sum_{\ell=0}^{T-1} \frac{ 1}{b_{\ell+1}}  \right)^2 \leq \frac{ \eta d LG^2 \log^2(1/\delta) }{2\varepsilon^2_{gen} }     \begin{cases} 
   \frac{1}{(1-p)}T^{2(1-p)} & p<1\\
\log^2(1+T) & p=1\\
\frac{1}{(p-1)^2}& p>1
\end{cases}
\end{align}
% \begin{align}
%  n^2  =  \frac{B_2}{B_1}\leq \frac{ d G^2 \log^2(1/\delta)     \left( \sum_{\ell=0}^{T-1} \frac{ 1}{b_{\ell+1}}  \right)^2       }{\varepsilon^2_{gen}\sum_{\ell=0}^{T-1} \frac{ \mathbb{E}[\|G_\ell\|^2]}{b^2_{\ell+1}} }\leq 
% \end{align}
\paragraph{Case 1:  $p=1/2$.}
Thus, we  have  from \eqref{eq:bound-optimal} %\eqref{eq:bound-general} that 
\begin{align}
 \sum_{\ell=0}^{T-1}  w_{\ell}\mathbb{E} \|\nabla L(\theta_\ell)\|^2\leq \frac{1}{n} \frac{\sqrt{\eta dL} G \log (1/\delta) }{\varepsilon_{gen} }   \sqrt{\frac{\mathbb{E}[L(\theta_{0})]}{\eta} +\frac{\eta L}{2}G^2\log(1+T) }  
\end{align}
To get the above bound, we require the complexity $T$ satisfying (by  \eqref{eq:n-square})
\begin{align}
 n^2 \varepsilon^2_{gen}  \leq 2dG^2\log^2(1/\delta) T /(\log(T)-1)
\end{align}
which means 
$T=\mathcal{O}\left( \frac{n^2 \varepsilon^2_{gen}(\log(T)-1) }{  d G^2 \log^2(1/\delta) }\right)$


\paragraph{Case 2:  $p=3/4$.}
Thus, we  have  from \eqref{eq:bound-optimal} %\eqref{eq:bound-general} that 
\begin{align}
 \sum_{\ell=0}^{T-1}  w_{\ell}\mathbb{E} \|\nabla L(\theta_\ell)\|^2\leq \frac{1}{n} \frac{\sqrt{\eta dL} G \log (1/\delta) }{\varepsilon_{gen} }   \sqrt{\frac{\mathbb{E}[L(\theta_{0})]}{\eta} +\eta LG^2 }  
\end{align}
To get the above bound, we require the complexity $T$ satisfying (by  \eqref{eq:n-square})
\begin{align}
 n^2 \varepsilon^2_{gen} &\leq \frac{ d G^2 \log^2(1/\delta)     \left( \sum_{\ell=0}^{T-1} \frac{ 1}{b_{\ell+1}}  \right)^2       }{\sum_{\ell=0}^{T-1} \frac{ \mathbb{E}[\|G_\ell\|^2]}{b^2_{\ell+1}} }  \\
&\leq  \frac{2dG^2\log^2(1/\delta) 4T^{1/2}}{4}
\end{align}
which means 
$T^{1/2}=\mathcal{O}\left( \frac{n^2 \varepsilon^2_{gen}}{  d G^2 \log^2(1/\delta) }\right)$



\paragraph{Case 3:  $p=1/3$.}
Thus, we  have  from \eqref{eq:bound-optimal} %\eqref{eq:bound-general} that 
\begin{align}
 \sum_{\ell=0}^{T-1}  w_{\ell}\mathbb{E} \|\nabla L(\theta_\ell)\|^2\leq \frac{1}{n} \frac{\sqrt{\eta dL} G \log (1/\delta) }{\varepsilon_{gen} }   \sqrt{\frac{\mathbb{E}[L(\theta_{0})]}{\eta} +\frac{3\eta L}{2}G^2T^{1/3} }  
\end{align}
To get the above bound, we require the complexity $T$ satisfying (by  \eqref{eq:n-square})
\begin{align}
 n^2 \varepsilon^2_{gen} &\leq \frac{ d G^2 \log^2(1/\delta)     \left( \sum_{\ell=0}^{T-1} \frac{ 1}{b_{\ell+1}}  \right)^2       }{\sum_{\ell=0}^{T-1} \frac{ \mathbb{E}[\|G_\ell\|^2]}{b^2_{\ell+1}} }  \\
&\leq  \frac{2dG^2\log^2(1/\delta) 4T^{4/3}}{3/2T^{1/3}}
\end{align}
which means 
$T=\mathcal{O}\left( \frac{n^2 \varepsilon^2_{gen}}{  d G^2 \log^2(1/\delta) }\right)$.
Thus the final bound is 
\begin{align}
 \sum_{\ell=0}^{T-1}  w_{\ell}\mathbb{E} \|\nabla L(\theta_\ell)\|^2\leq \frac{1}{n} \frac{\sqrt{\eta dL} G \log (1/\delta) }{\varepsilon_{gen} }   \sqrt{\frac{\mathbb{E}[L(\theta_{0})]}{\eta} +\frac{3\eta L}{2}G^2 \mathcal{O}\left( \frac{n^{2/3} \varepsilon^{2/3}_{gen}}{  d^{1/3} G^{2/3} \log^{2/3}(1/\delta) }\right) }  
\end{align}

Looks like large learning rate has not at all any benefit :(

\section{Some general approach to think about adaptive gradient method}
Assume
\begin{enumerate}
\item[A1] The random vectors $\xi_k$, $k = 0,1,2, \dots, $ are independent of each other and also of $x_k$;
% \item[A2] $\mathbb{E}_{\xi_k}[ \| G(x_k, \xi_k) -\nabla F(x_k) \|^2] \leq \sigma_G^2;$
\item[A2] $\| \nabla F(x) \|^2 \leq G^2$ uniformly.
\end{enumerate}
Let us think about the general update
% \begin{minipage}[t]{0.7\textwidth}
\begin{algorithm}[H]
\caption{\textbf{Private AdaGrad-Norm}}
\label{alg:privacy-ada2}
\begin{algorithmic}[1]
	    \State Input $\theta_0,b_t$,
	    \For {$ t=1,\ldots,T$} 
	      \State $\xi_t\sim \text{Uniform}(1,...,n)$  and $c_t\sim \mathcal{N}(0,\sigma I)$
	       \State $G_{t}= \nabla L(\theta_{t};x_{\xi_t})+{b'}_{t}c_t,$ 
	       	    \State update  parameter $b^2_{t+1}=b^2_{t}+\frac{1}{d\sigma^2} \|G_t\|^2$
	    \State update gradient $\theta_{t+1}=\theta_{t}-\eta  \frac{1}{b_{t+1}}G_t$

	    \EndFor
\end{algorithmic}
\end{algorithm}
% \begin{align}
%     b^2_{t+1} &=b^2_{t}+\frac{1}{b_t}\left( \|G_t\|^2-2\sqrt{b}_{t}\langle{G_t,c_t\rangle}\right)\\
%     &=b^2_{t}+\frac{1}{b_t}\left( \|\nabla L(\theta_{t};x_{\xi_t})\|^2+b_t-2\sqrt{b}_{t}\|c_t\|\langle{G_t,c_t\rangle}\right)
% \end{align}
% \end{minipage}
% \begin{minipage}[t]{0.5\textwidth}
% \begin{algorithm}[H]
% \caption{\textbf{Private adaptive learning rate}}
% \label{alg:privacy-ada-general} 
% \begin{algorithmic}[1]
% 	    \State Input $\theta_0,b_t$,
% 	    \For {$ t=1,\ldots,T$} 
% 	      \State $\xi_t\sim \text{Uniform}(1,...,n)$  and $c_t\sim \mathcal{N}(0,\sigma I)$
% 	    \State update $b_{t+1}$	 and $b'_{t+1}$ with certain rule    
% 	    \State update $\theta_{t+1}=\theta_{t}-  \frac{\eta}{b_{t+1}}(\nabla L(\theta_{t};x_{\xi_t})+b'_{t+1}c_t)$
% 	    \EndFor
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}

\begin{proof}
For simplicity, we write $F_j = F(\theta_j)$ and $\nabla F_j = \nabla F(\theta_j)$ and $\nabla F_{\xi_j} = \nabla F(\theta_j; x_{\xi_j})$.  By Decent Lemma \ref{lem:descend}, for $ j\geq 0,$
\begin{align}
F_{j+1} &\leq F_j - \eta\langle{ \nabla F_j,\frac{\nabla F_{\xi_j}}{b_{j+1}} +\frac{b_j'}{b_{j+1}}z_j\rangle}+\frac{ \eta  ^2 L}{2b^2_{j+1}} \|G_j\|^2 \nonumber 
\end{align}
Condition on $\xi_1, \dots, \xi_{j-1}$, we take expectation with respect to $\xi_{j}$, 
\begin{align}
\mathbb{E}_{\xi_j}[F_{j+1}] &=
\mathbb{E}_{\xi_j}[\mathbb{E}_{z_j}[F_{j+1}]]\\
&\overset{(a)}{\leq}  F_{j}-\frac{\eta}{b_{j}+\gamma_j}\langle{ \nabla F_j,\mathbb{E}_{\xi_j}[\nabla F_{\xi_j}+b_j'\mathbb{E}_{z_j}[z_j]]\rangle} +\mathbb{E}_{\xi_j}\left[\frac{ \eta ^2 L}{2b^2_{j+1}} \|G_{j}\|^2 +\left(\frac{\eta}{b_{j}+\gamma_j}-\frac{\eta}{b_{j+1}}\right)\langle{ \nabla F_j,G_j\rangle}\right] \nonumber \\
&\overset{(b)}{=}  F_{j}-\frac{\eta \| \nabla F_j\|^2}{b_{j}+\gamma_j}+\mathbb{E}_{\xi_j}\left[\frac{ \eta ^2 L}{2b^2_{j+1}} \|G_{j}\|^2 \right] +\mathbb{E}_{\xi_j}\left[\left(\frac{\eta}{b_{j}+\gamma_j}-\frac{\eta}{b_{j+1}}\right)\langle{ \nabla F_j,\nabla F_{\xi_j}+b_j'z_j\rangle}\right] \label{eq:adagrad1}
% & \quad + \left(\frac{ \eta ^2 L}{2} -\eta \right)\langle{ \nabla F_j, z_j\rangle}  +\frac{ \eta ^2 L}{2}\|z_j\|^2
\end{align}
where (a) is applied with $\gamma_j = \sqrt{G^2 + db'^2_j\sigma^2}$ and (b) follows from the fact of conditional expectation with respect to $z_{j}$  conditional on $\xi_1, \dots, \xi_{j-1},\xi_{j}$ gives
\begin{align}
\mathbb{E}_{z_j} \left[ z_j\right] &= 0  \text{ and }
\mathbb{E}_{\xi_j} \left[ \|z_j\|^2\right] = d\sigma^2
\end{align}
Applying telescoping to \eqref{eq:adagrad1} with $j=1,\ldots,T$, we get 
\begin{align}
\mathbb{E}\left[\sum_{j=0}^{T-1}\frac{\| \nabla F_j\|^2}{b_{j}+\gamma_j}\right]
&\leq \frac{F_{0}}{\eta}+ \mathbb{E} \left[\sum_{j=0}^{T-1}\frac{ \eta  L}{2b^2_{j+1}} \|G_{j}\|^2 \right]
+\mathbb{E} \left[\sum_{j=0}^{T-1}\mathbb{E}_{\xi_j}\left[\frac{b_{j+1}-b_j-\gamma_j}{b_{j+1}(b_{j}+\gamma_j)}\langle{ \nabla F_j,\nabla F_{\xi_j}+b_j'z_j\rangle}\right] \right] \label{eq:adagrad2}
% & \quad + \left(\frac{ \eta ^2 L}{2} -\eta \right)\langle{ \nabla F_j, z_j\rangle}  +\frac{ \eta ^2 L}{2}\|z_j\|^2
\end{align}



Now, observe the identity 
$$
\frac{b_{j+1}-b_j-\gamma_j}{b_{j+1}(b_{j}+\gamma_j)}  = \frac{ \|G_j\|^2/(d\sigma^2)}{b_{j+1}(b_{j}+\gamma_j)(b_{j}+b_{j+1})}-\frac{\gamma_j}{b_{j+1}(b_{j}+\gamma_j)};
$$
thus, applying Cauchy-Schwarz,
\begin{align}
\frac{b_{j+1}-b_j-\gamma_j}{b_{j+1}(b_{j}+\gamma_j)} \langle{ \nabla F_{j}, G_{j}\rangle}
&
= \left(\frac{\|G_j\|^2/(d\sigma^2)}{b_{j+1}(b_{j}+\gamma_j)(b_{j+1}+b_j)}-\frac{\gamma_j}{b_{j+1}(b_{j}+\gamma_j)}\right) \langle{ \nabla F_{j}, G_{j}\rangle}
\nonumber \\
&\leq 
\frac{ \|G_j\|^2 \|G_j\| \nabla F_{j}\|/(d\sigma^2)}{b_{j+1}(b_{j+1}+b_{j})(b_{j}+\gamma_j)} + \frac{\gamma_j|\langle{ \nabla F_{j}, G_{j}\rangle}|}{b_{j+1}(b_{j}+\gamma_j)} 
\nonumber \\
&\leq
\frac{ \|G_j\| \|G_j\| \nabla F_{j}\|/(d\sigma^2)}{(b_{j+1}+b_{j})(b_{j}+\gamma_j)} +\frac{\gamma_j\| \nabla F_{j}\|\| G_{j}\|}{b_{j+1}(b_{j}+\gamma_j)} 
\label{eq:key-inq1}
\end{align}

By applying the inequality  $ a b \leq \frac{\lambda }{2}a^2 + \frac{1}{2\lambda} b^2$  with $\lambda=\frac{2\gamma_j^2}{b_{j}+\gamma_j}$, $a=\frac{\|G_j\|}{b_{j}+b_{j+1}}$, and $b= \frac{\|\nabla F_j\| \|G_j\| }{(b_{j}+\gamma_j)}$, the first term in \eqref{eq:keyinq1} can be bounded as
\begin{align}
 \mathbb{E}_{\xi_j}\frac{\|G_{j}\|^2\| \nabla F_{j}\| }{(b_{j}+b_{j+1})(b_{j}+\gamma_j)} 
 & \leq 
  \mathbb{E}_{\xi_j}  \frac{\gamma_j ^2}{(b_{j}+\gamma_j)}\frac{\|G_j\|^2}{(b_{j}+b_{j+1})^2}
   + \mathbb{E}_{\xi_{j}} \frac{(b_{j}+\gamma_j)}{4\gamma_j^2}\frac{  \|\nabla F_{j}\|^2 \| G_{j}\|^2}{(b_{j}+\gamma_j)^2} 
   \nonumber \\ 
 &\leq    \frac{\gamma_j ^2}{b_{j}+\gamma_j}\mathbb{E}_{\xi_j} \left[ \frac{\|G_j\|^2}{b_{j+1}^2} \right] +  \frac{(b_{j}+\gamma_j)}{4\gamma_j^2}\frac{  \|\nabla F_{j}\|^2 \mathbb{E}_{\xi_{j}} \left[ \| G_{j}\|^2 \right]}{(b_{j}+\gamma_j)^2} \nonumber \\ 
  & \overset{(a)}{\leq}  \gamma_j\mathbb{E}_{\xi_j} \left[ \frac{\|G_j\|^2}{b_{j+1}^2} \right] +  \frac{ \|\nabla F_{j}\|^2}{4(b_{j}+\gamma_j)} \label{eq:keyinq_a1}
\end{align}
where  (a) follows from the fact that $ \mathbb{E}_{\xi_{j}} \left[ \| G_{j}\|^2\right] =  \mathbb{E}_{\xi_{j}} \left[ \| \nabla F_{\xi_j}\|^2 + b_j'^2\| z_{j}\|^2 \right] \leq G^2+d b_j'^2\sigma^2=\gamma_j$. 
Similarly, applying the inequality  $a b \leq \frac{\lambda}{2} a^2 + \frac{1}{2\lambda} b^2$  with $\lambda=\frac{2}{b_{j}+\gamma_j}$, $a=\frac{\gamma_j\|G_j\|}{b_{j+1}}$, and $b= \frac{\|\nabla F_j\| }{b_{j}+\gamma_j}$, the second term of the right hand side in  \eqref{eq:key-inq1} is bounded by
\begin{align}
 \mathbb{E}_{\xi_j}\frac{\gamma_j\| \nabla F_{j}\|\| G_{j}\|}{b_{j+1}(b_{j}+\gamma_j)}  
 & \leq  \gamma_j \mathbb{E}_{\xi_{j}} \frac{\|G_{j}\|^2}{b_{j+1}^2}+ \frac{  \|\nabla F_{j}\|^2}{4(b_{j}+\gamma_j)} \leq  \gamma_j \mathbb{E}_{\xi_{j}} \frac{\|G_j\|^2}{b_{j+1}^2}+ \frac{  \|\nabla F_{j}\|^2}{4(b_{j}+\gamma_j)}. \label{eq:keyinq_a2}
\end{align}
Thus, combing \eqref{eq:keyinq_a1} and \eqref{eq:keyinq_a2}, we have
\begin{align}
 \mathbb{E}_{\xi_j} \left[  \frac{b_{j+1}-b_j-\gamma_j}{b_{j+1}(b_{j}+\gamma_j)} \langle{ \nabla F_j, G_j \rangle} \right] 
&\leq \frac{2\gamma_j}{d\sigma^2}\mathbb{E}_{\xi_j} \left[ \frac{\|G_j\|^2}{b_{j+1}^2} \right] +  \frac{\|\nabla F_{j}\|^2}{2(b_{j}+\gamma_j)} 
\end{align}
and, therefore back to \eqref{eq:adagrad2} with $\gamma_j = \sqrt{G^2 + db'^2_j\sigma^2}$
\begin{align}
\mathbb{E}\left[\sum_{j=0}^{T-1}\frac{\| \nabla F_j\|^2}{2(b_{j}+\gamma_j)}\right]
&\leq \frac{F_{0}}{\eta}+  \mathbb{E} \left[\sum_{j=0}^{T-1}\left(\frac{\eta L}{2}+\frac{2\gamma_j}{d\sigma^2} \right)\frac{\|G_{j}\|^2}{b^2_{j+1}}  \right] \label{eq:key-telescope}\\
&\leq \frac{F_{0}}{\eta}+  \mathbb{E} \left[\sum_{j=0}^{T-1}\left(\frac{\eta L}{2}+\frac{2G }{d\sigma^2}  + \frac{b_j'^2}{\sqrt{d}\sigma}\right)\frac{\|G_{j}\|^2}{b^2_{j+1}}  \right]
\end{align}

Observe $b^2_{t+1}=b^2_{t}+\frac{1}{d\sigma^2} \|G_t\|^2=b_0^2+\frac{1}{d\sigma^2}\sum_{\tau=0}^{t} \|G_\tau\|^2$ 

\begin{align}
\sum_{j=0}^{T-1}\frac{ \|G_{j}\|^2}{b^2_{j+1}} 
% &=\sum_{j=0}^{T-1}\frac{d\sigma^2 \|G_{j}\|^2 }{b^2_{0}d\sigma^2+\sum_{\tau=0}^{j} \|G_\tau\|^2} \\
&=d\sigma^2\sum_{j=0}^{T-1}\frac{\|G_{j}\|^2/(b^2_{0}d\sigma^2) }{1+\sum_{\tau=0}^{j} \|G_\tau\|^2/(b^2_{0}d\sigma^2)} \leq d\sigma^2+d\sigma^2 \log\left( 1+\sum_{\tau=0}^{T-1} \frac{\|G_\tau\|^2}{b^2_{0}d\sigma^2} \right) \\
\mathbb{E} \left[\sum_{j=0}^{T-1}\frac{ \|G_{j}\|^2}{b^2_{j+1}} \right] 
&\leq d\sigma^2+d\sigma^2 \log\left( 1+\sum_{\tau=0}^{T-1} \frac{\mathbb{E} \left[\|G_\tau\|^2\right]}{b^2_{0}d\sigma^2} \right) \leq d\sigma^2+d\sigma^2 \log\left( 1+\frac{TG^2+d\sigma^2\sum_{j=0}^{T-1}b_j'^2}{b^2_{0}d\sigma^2} \right) \label{eq:final-eq1}
\end{align}
Note also that
$\mathbb{E}\left[b_{t+1}^2\right] = b_0^2+ \frac{1}{d\sigma^2 }\sum_{j=0}^{t}\left(\mathbb{E}\left[\| \nabla F_j\|^2\right] +  db'^2_j\sigma^2\right).
$ Then the left hand side of \eqref{eq:key-telescope}, we have
\begin{align}
  \mathbb{E}\left[ \sum_{j=0}^{T-1} \frac{\| \nabla F_j\|^2}{b_j +\gamma_j} \right] 
  &\geq \sum_{j=0}^{T-1}\mathbb{E}\left[\frac{\| \nabla F_j\|^2}{\sqrt{b^2_{0}+ \frac{1}{d\sigma^2}\sum_{\tau=0}^{j} \|G_\tau\|^2+\gamma_j^2}}\right] \\
  &\geq   \sum_{j=0}^{T-1}\frac{\mathbb{E}\left[\| \nabla F_j\|^{4/3}\right]^{3/2}}{\sqrt{b_{0}^2+\frac{1}{d\sigma^2}\sum_{\tau=0}^{j}\mathbb{E}\left[\|G_\tau\|^2\right]+\gamma_j^2}} \\
    &=    \sum_{j=0}^{T-1}\frac{\mathbb{E}\left[\| \nabla F_j\|^{4/3}\right]^{3/2}}{\sqrt{b_{0}^2+\sum_{\tau=0}^{j}\left(b'^2_\tau+\frac{\mathbb{E}\left[\|\nabla F_\tau\|^2\right]}{d\sigma^2}\right)+\gamma_j^2}}\\
    &=    \sum_{j=0}^{T-1}\frac{\mathbb{E}\left[\| \nabla F_j\|^{4/3}\right]^{3/2}}{\sqrt{b_{0}^2+\sum_{\tau=0}^{j}\left(b'^2_\tau+\frac{\mathbb{E}\left[\|\nabla F_\tau\|^2\right]}{d\sigma^2}\right)+\gamma_j^2}}
\end{align}



















\end{proof}











\section{Privacy Guarantee for Algorithm \ref{alg:privacy1} (version 2)}
\begin{prop}
Let $Z\sim\mathcal{N}(0,\sigma_z^2)$. At iteration $t$, we have the privacy mechanism $\mathcal{M}_t:\mathbb{R}^d\to\mathbb{R}^d$ for $f_t(X)=\nabla L(\theta_t;x_{\xi_t})$  with $x_{\xi_t}\sim X$ :
%some $f(X):\mathbb{R}\to\mathbb{R}$ and $b(X):\mathbb{R}\to\mathbb{R}$ follows
\[\mathcal{M}^{\text{SGD}}_t(X)=\frac{f_t(X)}{\sqrt{b_0+tc_b}}+Z.\]
\end{prop}

Define the distance $\Delta_t^{\text{SGD}} = \left\| \frac{f_t(X')-f_t(X)}{\sqrt{b_t^2+tc_b}} \right\|^2$. % \|\frac{f_t(X)}{\sqrt{b_t^2(X)+f_t^2(X)}}-\frac{f_t(X')}{\sqrt{b_t^2(X')+\|f_t(X')\|^2}}\|^2$ 
The upper bound of  $\Delta_t^{\text{AG}}$ is % the the norm different between $M(X)$ and $M(X')$
\begin{align}
 \Delta^{\text{SGD}}_t 
  &\leq\frac{ \left\|f_t(X')-f_t(X)\right\|^2}{\sqrt{b_0^2+tc_b}}
\end{align}
The supreme of $\Delta_t^{\text{SGD}}$  over the iterations ${f_t(X)}$ and ${f_t(X)}$ is
\begin{align}
\sup_{X,X'} \Delta^{\text{SGD}}_t \leq \frac{G^2}{\sqrt{b_0^2+tc_b}}
\end{align}
Thus, by Lemma \ref{lem:gaussian} and  privacy by amplification, $\mathcal{M}_t^{\text{AG}}$ at $t$ iteration is $(\varepsilon_t, \delta_t)-$DP if  $Z\sim \mathcal{N}(0,\sigma_z)$ where
\begin{align}
  \varepsilon_t  \leq \frac{ \sqrt{2\ln(1.25/\delta_t)}}{ n\sigma_z}\sqrt{\frac{ G^2}{{b_0^2+t c_b}} } 
\end{align}
Let $\delta_0=\delta_2=\ldots=\delta_t$. Using  extended advanced composition \ref{thm:advanced-comp}, we have the final output follow $(\varepsilon_{SGD}, \delta_{\text{SGD}})-DP$ where 

 \begin{align}
   \varepsilon_{SGD} &= \sqrt{\sum_{t=0}^{T-1} \varepsilon_t^2 \log\left(\frac{1}{\delta'}\right)} +  \sum_{i=1}^K \frac{\varepsilon_t^2}{2+\varepsilon_t} \\
   &\leq 2\sqrt{\sum_{t=0}^{T-1} \varepsilon_t^2 \log\left(\frac{1}{\delta'}\right)}\\
   &\leq \frac{2\sqrt{2\log\left({1}/{\delta'}\right)\log\left({1.25}/{\delta_0}\right)}}{n  \sigma_z} \sqrt{\sum_{t=1}^{T-1}  \frac{ G^2}{b_0+t c_b}  }      \\
   &= \frac{2G\sqrt{2\log\left({1}/{\delta'}\right)\log\left({1.25}/{\delta_0}\right)}}{n \sigma_z} \sqrt{\frac{ 1}{c_b}\sum_{t=1}^{T-1}  \frac{1}{b_0/c_b+t} }    \\
      &\leq \frac{2G\sqrt{2\log\left({1}/{\delta'}\right)\log\left({1.25}/{\delta_0}\right)}}{n \sigma_z} \sqrt{\frac{1}{b_0}+\frac{1}{c_b}\log \left(\frac{b_0+Tc_b}{b_0}\right)}  \\
  &= \mathcal{O}\left( \frac{G\sqrt{\log\left({1}/{\delta'}\right)\log\left({1}/{\delta_0}\right)}}{n \sigma_z} \sqrt{\frac{1}{b_0}+\frac{\log(1+Tc_b/b_0)}{c_b}}     \right)
\end{align}
Here, in the first inequality, the term $\sum_{i=1}^K \frac{\varepsilon_t^2}{2+\varepsilon_t}$ is considerable smaller  than $\sqrt{\sum_{t=0}^{T-1} \varepsilon_t^2 \log\left(\frac{1}{\delta_0}\right)}$. In addition,
\begin{align}
\delta_{\text{SGD}} &= 1 - (1- \delta_0) (1- \delta_1)(1-\delta_2) \hdots (1-\delta_{T-1}) + \delta' 
   = 1 - (1- \delta_0)^T + \delta' \leq \delta'
\end{align}
This implies that 
\begin{align}
    \varepsilon_{SGD} = \mathcal{O}\left( \frac{G\sqrt{\log\left({1}/\delta_{\text{SGD}}\right)\log\left({1}/{\delta_0}\right)}}{n \sigma_z} \sqrt{\frac{\log(T)}{c_b}}     \right)
\end{align}


\begin{align}
    \varepsilon_{SGD} = \mathcal{O}\left( \frac{G \log\left({1}/{\delta_{SGD}}\right)}{n \sigma_z} \sqrt{\frac{\log(T)}{c_b}}     \right)
\end{align}
\subsection{Convergence}
Assume
\begin{enumerate}
\item[A1] The random vectors $\xi_k$, $k = 0,1,2, \dots, $ are independent of each other and also of $x_k$;
% \item[A2] $\mathbb{E}_{\xi_k}[ \| G(x_k, \xi_k) -\nabla F(x_k) \|^2] \leq \sigma_G^2;$
\item[A2] $\| \nabla F(x) \|^2 \leq G^2$ uniformly.
\end{enumerate}
Recall the update in Algorithm \ref{alg:privacy-ada2}:
\begin{align*}
\theta_{t+1}&= \theta_t - \eta \frac{\eta g_{\xi_t}}{\sqrt{b^2_{0}+ tc_b}}+ \eta Z
\end{align*}
By Lipschitz gradient smoothness:
\begin{align}
L(\theta_{j+1}) &\leq L(\theta_{j}) - \eta\langle{ \nabla L(\theta_j),\frac{ g_{\xi_j}}{\sqrt{b^2_{0}+ tc_b}} +z_j\rangle}+\frac{ \eta^2 L}{2} \left\| \frac{ g_{\xi_j}}{\sqrt{b^2_{0}+ tc_b}}+  z_j  \right\|^2 \nonumber \\
\mathbb{E}[L(\theta_{j+1})] &\leq \mathbb{E}[L(\theta_{j})] -\frac{ \eta \mathbb{E}[\|\nabla L(\theta_{j})\|^2]}{\sqrt{b^2_{0}+ tc_b}} +\frac{ \eta ^2 L}{2(b_{0}+ tc_b)} \mathbb{E}[\|g_{\xi_j}\|^2]  +\frac{ \eta ^2 d L \sigma_z^2}{2} % \label{remark2}
\end{align}
So we have%think about $\eta_t = \frac{\eta}{\sqrt{b^2_{0}+ tc_b}}$
\begin{align*}
 \frac{ 1}{\sqrt{b_0^2+ Tc_b}} \sum_{\ell=0}^{T-1}\mathbb{E}  \|\nabla L(\theta_\ell)\|^2
   & \leq \sum_{\ell=0}^{T-1}\frac{\mathbb{E}  \|\nabla L(\theta_\ell)\|^2}{\sqrt{b_0^2+\ell c_b}} 
    \leq  \frac{\mathbb{E}[L(\theta_{0})]  }{\eta}+ \frac{\eta G^2 L}{2}\sum_{\ell=0}^{T-1} \frac{1}{b_0+ tc_b}  +\frac{ \eta dT L \sigma_z^2}{2}  \\
   \Rightarrow \frac{1}{T}\sum_{\ell=0}^{T-1}\mathbb{E}  \|\nabla L(\theta_\ell)\|^2
   & \leq  \frac{\sqrt{b_0^2+ Tc_b}\mathbb{E}[L(\theta_{0})]  }{T \eta}+ \frac{\eta G^2 L\sqrt{b_0^2+ Tc_b}}{2b_0T}\left(1+\frac{b_0\log(1+Tc_b/b_0)}{c_b}\right)  +\frac{ \eta d\sqrt{b_0^2+ Tc_b} L \sigma_z^2}{2}  \\
   & =\mathcal{O}\left(\frac{\sqrt{c_b}}{ \eta \sqrt{T}}\right) + \mathcal{O}\left(\frac{\eta G^2 L\log(1+Tc_b/b_0)}{ \sqrt{Tc_b}}\right)  +\frac{ \eta d\sqrt{b_0^2+ Tc_b} L}{2} \frac{G^2 \log^2\left({1}/{\delta_{SGD}}\right)}{n^2 \varepsilon^2_{SGD}} \frac{\log(T)}{c_b}   \\   
\end{align*}





% \begin{remark}
% Compare with Standard SGD

% % $\eta =\mathcal{O} \left(\frac{1}{\sqrt{t}}\right)$


% \end{remark}


\section{Privacy Guarantee for Algorithm \ref{alg:privacy-ada2} (version 3)}
\begin{prop}
Let $Z\sim\mathcal{N}(0,\sigma_z^2)$. At iteration $t$, we have the privacy mechanism $\mathcal{M}_t:\mathbb{R}^d\to\mathbb{R}^d$ for $f_t(X)=\nabla L(\theta_t;x_{\xi_t})$  with $x_{\xi_t}\sim X$ :
%some $f(X):\mathbb{R}\to\mathbb{R}$ and $b(X):\mathbb{R}\to\mathbb{R}$ follows
\[\mathcal{M}^{\text{AG}}_t(X)=\frac{f_t(X)}{\sqrt{b_t^2(X)+\|f_t(X)\|^2}}+Z\]
where    $b_t^2(X) = b_0^2+\sum_{k=1}^{t-1}\max{\{\| \nabla L(\theta_k;x_{\xi_k})\|^2,\varepsilon\}} $ for Algorithm \ref{alg:privacy-ada2}.
\end{prop}

The proof of the proposition is straight forward for the above mechanism for Algorithm \ref{alg:privacy-ada2} at iteration $t$.
Define the distance $\Delta_t^{\text{AG}} = \left\| \frac{f_t(X)}{\sqrt{b_t^2(X)+\max{ \{\|f_t(X)\|^2,c_b\}}}}- \frac{f_t(X')}{\sqrt{b_t^2(X')+\max{\{\|f_t(X')\|^2,c_b\}}}} \right\|^2$. % \|\frac{f_t(X)}{\sqrt{b_t^2(X)+f_t^2(X)}}-\frac{f_t(X')}{\sqrt{b_t^2(X')+\|f_t(X')\|^2}}\|^2$ 
The upper bound of  $\Delta_t^{\text{AG}}$ is % the the norm different between $M(X)$ and $M(X')$
\begin{align}
 \Delta^{\text{AG}}_t 
  &\leq\frac{ 2\left\| f_t(X)\right\|^2}{{b_t^2(X)+\max{ \{\|f_t(X)\|^2,c_b\}}}}+ \frac{2\left\|f_t(X')\right\|^2}{{b_t^2(X')+\|f_t(X')\|^2+\varepsilon}} \\
   &\leq \frac{ 2\left\| f_t(X)\right\|^2}{{b_0^2+\sum_{k=0}^{t-1} \max{\{\|f_k(X)\|^2,  c_b\}}+\|f_t(X)\|^2}}+ \frac{2\left\|f_t(X')\right\|^2}{{b_0^2+\sum_{k=0}^{t-1} \max{\{\|f_k(X')\|^2,c_b\}}+\|f_t(X')\|^2}} 
\end{align}
The supreme of $\Delta_t^{\text{AG}}$ and $ \sum_{t=0}^{T-1}\Delta_t^{\text{AG}}$ over the iterations ${f_t(X)}$ and ${f_t(X)}$ is
\begin{align}
\sup_{X,X'} \Delta^{\text{AG}}_t 
            %   &\leq \sup_{t,X,X'} \frac{ 2\left\| f_t(X)\right\|^2}{{b_t^2(X)+\max{ \{\|f_t(X)\|^2,c_b\}}}}+ \sup_{t,X,X'}\frac{2\left\|f_t(X')\right\|^2}{{b_t^2(X')+\|f_t(X')\|^2+\varepsilon}} \\
%   &=\sup_{t,X,X'}\frac{ 2\left\| f_t(X)\right\|^2}{{b_0+\sum_{k=0}^{t}\|f_k(X)\|^2+(t+1)\varepsilon}}+ \sup_{t,X,X'}\frac{2\left\|f_t(X')\right\|^2}{{b_0+\sum_{k=0}^{t}\|f_k(X)\|^2+(t+1)\varepsilon}} \\
   &\leq \sup_{t,X,X'}\frac{ 2\left\| f_t(X)\right\|^2}{{b_0^2+\sum_{k=0}^{t-1} \max{\{\|f_k(X)\|^2,  c_b\}}+\|f_t(X)\|^2}}+ \sup_{t,X,X'}\frac{2\left\|f_t(X')\right\|^2}{{b_0^2+\sum_{k=0}^{t-1} \max{\{\|f_k(X')\|^2,c_b\}}+\|f_t(X')\|^2}} \nonumber\\
 &\leq \sup_{X,X'}\frac{ 2G^2}{{b_0^2+\sum_{k=0}^{t-1} \max{\{\|f_k(X)\|^2,  c_b\}}+G^2}}+ \sup_{t,X,X'}\frac{2G^2}{{b_0^2+\sum_{k=0}^{t-1} \max{\{\|f_k(X')\|^2,c_b\}}+G^2}} \nonumber\\
%   &\leq \sup_{t,X,X'}\frac{ 2G^2}{{b_0^2+\sum_{k=0}^{t-1} \max{\{\|f_k(X)\|^2,  c_b\}}+G^2}}+ \sup_{t,X,X'}\frac{2G^2}{{b_0^2+\sum_{k=0}^{t-1} \max{\{\|f_t(X')\|^2,\varepsilon\}}+G^2}} \nonumber\\
 &\leq \frac{ 4G^2}{{b_0^2+t c_b+G^2}}  \nonumber
\end{align}
Thus, by Lemma \ref{lem:gaussian} and  privacy by amplification, $\mathcal{M}_t^{\text{AG}}$ at $t$ iteration is $(\varepsilon_t, \delta_t)-$DP if  $Z\sim \mathcal{N}(0,\sigma_z)$ where
\begin{align}
  \varepsilon_t  \leq \frac{ \sqrt{2\ln(1.25/\delta_t)}}{ n\sigma_z}\sqrt{\frac{ 4G^2}{{b_0^2+G^2+t c_b}} } 
\end{align}
Let $\delta_0=\delta_2=\ldots=\delta_t$. Using  extended advanced composition \ref{thm:advanced-comp}, we have the final output follow $(\varepsilon_{SGD}, \delta_{\text{AG}})-DP$ where 

 \begin{align}
   \varepsilon_{SGD} &= \sqrt{\sum_{t=0}^{T-1} \varepsilon_t^2 \log\left(\frac{1}{\delta'}\right)} +  \sum_{i=1}^K \frac{\varepsilon_t^2}{2+\varepsilon_t} \\
   &\leq 2\sqrt{\sum_{t=0}^{T-1} \varepsilon_t^2 \log\left(\frac{1}{\delta'}\right)}\\
   &\leq \frac{2\sqrt{2\log\left({1}/{\delta'}\right)\log\left({1.25}/{\delta_0}\right)}}{n  \sigma_z} \sqrt{  \frac{ 4G^2}{b_0^2+G^2}+\sum_{t=1}^{T-1}  \frac{ 4G^2}{b_0^2+G^2+t c_b}  }      \\
   &= \frac{4G\sqrt{2\log\left({1}/{\delta'}\right)\log\left({1.25}/{\delta_0}\right)}}{n \sigma_z} \sqrt{ \frac{1}{b_0^2+G^2}+\frac{ 1}{c_b}\sum_{t=1}^{T-1}  \frac{1}{(b_0^2+G^2)/c_b+t} }    \\
      &\leq \frac{4G\sqrt{2\log\left({1}/{\delta'}\right)\log\left({1.25}/{\delta_0}\right)}}{n \sigma_z} \sqrt{\frac{1}{b_0^2+G^2}+\frac{1}{c_b}\log \left(\frac{(b_0^2+G^2)/c_b+T}{(b_0^2+G^2)/c_b}\right)}  \\
  &= \mathcal{O}\left( \frac{G\sqrt{\log\left({1}/{\delta'}\right)\log\left({1}/{\delta_0}\right)}}{n \sigma_z} \sqrt{\frac{\log(T)}{c_b}}     \right)
\end{align}
Here, in the first inequality, the term $\sum_{i=1}^K \frac{\varepsilon_t^2}{2+\varepsilon_t}$ is considerable smaller  than $\sqrt{\sum_{t=0}^{T-1} \varepsilon_t^2 \log\left(\frac{1}{\delta_0}\right)}$. In addition,
\begin{align}
\delta_{\text{AG}} &= 1 - (1- \delta_0) (1- \delta_1)(1-\delta_2) \hdots (1-\delta_{T-1}) + \delta' 
   = 1 - (1- \delta_0)^T + \delta' \leq \delta'
\end{align}
This implies that 
\begin{align}
    \varepsilon_{SGD} = \mathcal{O}\left( \frac{G\sqrt{\log\left({1}/\delta_{\text{AG}}\right)\log\left({1}/{\delta_0}\right)}}{n \sigma_z} \sqrt{\frac{\log(T)}{c_b}}     \right)
\end{align}


\begin{align}
    \varepsilon_{SGD} = \mathcal{O}\left( \frac{G \log\left({1}/{\delta}\right)}{n \sigma_z} \sqrt{\frac{\log(T)}{c_b}}     \right)
\end{align}
\subsection{Convergence}
Assume
\begin{enumerate}
\item[A1] The random vectors $\xi_k$, $k = 0,1,2, \dots, $ are independent of each other and also of $x_k$;
% \item[A2] $\mathbb{E}_{\xi_k}[ \| G(x_k, \xi_k) -\nabla F(x_k) \|^2] \leq \sigma_G^2;$
\item[A2] $\| \nabla F(x) \|^2 \leq G^2$ uniformly.
\end{enumerate}
Recall the update in Algorithm \ref{alg:privacy-ada2}:
\begin{align*}
    \theta_{t+1}
    &= \theta_t - \eta \left( \frac{ g_{\xi_t}}{\sqrt{b^2_{0}+ \sum_{k=0}^t\{\| g_{\xi_k}\|^2,c_b\}}} + Z\right) 
\end{align*}

\begin{thm}\label{thm:adagrad-version3}
    
\end{thm}


For non-convex function, we get (see the proof in Appendix \ref{sec:proof-adagrad-version4})
\begin{align}
   \min_{\ell=0,1,\dots, N-1} \left( \mathbb{E}  \|\nabla L_{\ell}(\theta_\ell; X)\|^{
   \frac{4}{3}} \right)^\frac{3}{2}  &\leq \left( \frac{2\sqrt{2}b_0}{N} + \frac{\sqrt{2}\gamma}{\sqrt{N}}\right)\left(  \frac{ F_{0} - F^{*} }{\eta}+ \left(2\gamma + \frac{\eta L}{2}\right) \log \left( \frac{N\gamma^2}{b_0^2} +1  \right) 
 \right) \nonumber\\
 &+\frac{\left(\sqrt{2N\gamma^2+2b_0^2} + \sqrt{2}{b_0} \right)\eta L d\sigma_z^2 }{2}   
 \end{align}
 To simplify
  \begin{align}
   \min_{\ell=0,1,\dots, N-1} \left( \mathbb{E}  \|\nabla L_{\ell}(\theta_\ell; X)\|^{
   \frac{4}{3}} \right)^\frac{3}{2}  &=\mathcal{O}\left(  \frac{\gamma(\gamma +\eta L)\log(N)}{\sqrt{N}}\right) +  \mathcal{O}\left(  (\gamma\sqrt{N} +b_0)\eta Ld \sigma_z^2\right) \\
  &=\mathcal{O}\left(  \frac{\gamma(\gamma +\eta L)\log(N)}{\sqrt{N}}\right) +  \mathcal{O}\left(  (\gamma\sqrt{N} +b_0)\eta Ld  \frac{G^2\log\left({1}/{\delta_0}\right)}{n^2 \varepsilon_{SGD}^2} \frac{\log(N)}{c_b} \right) \\
    &=\widetilde {\mathcal{O}}\left(  \frac{1}{\sqrt{N}}\right) +  \widetilde {\mathcal{O}}\left(  \frac{\sqrt{N}}{n^2}  \right)
  %  &+\frac{\left(\sqrt{2N\gamma^2+2b_0^2} + \sqrt{2}{b_0} \right)\eta L d}{2}  \frac{4G\sqrt{2}\log\left({1.25}/{\delta_0}\right)}{n \varepsilon} \frac{1}{b_0^2+G^2}+\frac{1}{}\log \left(\frac{(b_0^2+G^2)/\varepsilon+N}{(b_0^2+G^2)/\varepsilon}\right)    \\
\end{align}
To find the optimal $N$, we let the left hand side equal to right hand side, we get 
$N=\Theta\left( n^2\right)$ and so 
 \begin{align}
   \min_{\ell=0,1,\dots, N-1} \left( \mathbb{E}  \|\nabla L_{\ell}(\theta_\ell; X)\|^{
   \frac{4}{3}} \right)^\frac{3}{2}  &=\mathcal{O}\left(\frac{1}{n} \right)
\end{align}



\begin{remark}
Compare with Standard SGD
\begin{align*}
   \min_{\ell=0,1,\dots, N-1} \mathbb{E}  \|\nabla L_{\ell}(\theta_\ell; X)\|^2
   &\leq    \frac{\|\nabla L_{0}(\theta_0; X)\|^2}{ \sum_{k=0}^{N-1} \eta_k} +\frac{\sum_{k=0}^{N-1} \eta_k^2\left( \gamma^2 L +d\sigma_z^2 \right) }{\sum_{k=0}^{N-1} \eta_k} \\
  &\leq    \mathcal{O}\left( \frac{\sum_{k=0}^{N-1} \eta_k^2\left( \gamma^2 L \right) }{\sum_{k=0}^{N-1} \eta_k} \right)+\mathcal{O}\left( \frac{d\sigma_z^2  \sum_{k=0}^{N-1} \eta_k^2 }{\sum_{k=0}^{N-1} \eta_k} \right)\\
    &\leq    \mathcal{O}\left( \frac{ \gamma^2 L\log(N) }{\sqrt{N}} \right)+\mathcal{O}\left( \frac{d \log(N) }{\sqrt{N}}\sigma_z^2  \right)\\
    %   &\leq    \mathcal{O}\left( \frac{ \gamma^2 L\log(N) }{\sqrt{N}} \right)+\mathcal{O}\left( \frac{d \log(N) }{\sqrt{N}}  \right)
    &\leq    \mathcal{O}\left( \frac{ \gamma^2 L\log(N) }{\sqrt{N}} \right)+\mathcal{O}\left( \frac{d\log(N) }{\sqrt{N}} \frac{N\log(1/\delta)  }{n^2\varepsilon^2_{\text{GD}}}\right)
\end{align*}
% $\eta =\mathcal{O} \left(\frac{1}{\sqrt{t}}\right)$


\end{remark}




% Let the density function of $\mathcal{M}(x)$ be $f_{\mathcal{M}(x)}(y)$.
% Define the privacy loss function $\mathcal{L}_{\mathcal{M}}^{x,x'}(y)$ and privacy loss random variable  $L_{\mathcal{M}}^{x,x'}$ as follows
% \begin{align}
% \mathcal{L}_{\mathcal{M}}^{x,x'}(y) &=\ln\left( \frac{f_{\mathcal{M}(x)}(y)}{f_{\mathcal{M}(x')}(y)} \right) \label{eq:privacy-def}; \quad  L_{\mathcal{M}}^{x,x'}= \mathcal{L}_{\mathcal{M}}^{x,x'}( \mathcal{M}(x)). 
% \end{align}




\section{Privacy Guarantee for Algorithm \ref{alg:privacy-ada} (version 1)}
% \begin{minipage}[t]{0.5\textwidth}
\begin{algorithm}[H]
\caption{\textbf{Private AdaGrad-Norm} (version 1)}
\label{alg:privacy-ada}
\begin{algorithmic}[1]
	    \State Input $\theta_0,b_t$,
	    \For {$ t=1,\ldots,T$} 
      \State update $b^2_{t+1}=b^2_{t}+\|\nabla L(\theta_{t};x_{\xi_t})\|^2$
	    \State $G_{t}= \nabla L(\theta_{t};x_{\xi_t})+c_t,$ where
	    
	    $\xi_t\sim \text{Uniform}(1,...,n)$  and $c_t\sim \mathcal{N}(0,\sigma I)$

	    \State update $\theta_{t+1}=\theta_{t}-\frac{\eta}{b_{t+1}}G_t$
	    \EndFor
\end{algorithmic}
\end{algorithm}
% \end{minipage}
The proof for this section follow the tutorial given in \url{https://simons.berkeley.edu/talks/large-scale-private-learning}.
% \me{Amplification by iteration}
Observe the update of Algorithm  \ref{alg:privacy-ada} (AdaGrad) is 
\begin{align}
    \theta_{t+1}=\theta_t- \frac{ \eta G_t}{\sqrt{b_0^2+\sum_{i=1}^t \|G_{i}\|^2}}=\theta_{t-1}- \frac{ \eta (g_{\xi_t}+c_t)}{\sqrt{b_0^2+\sum_{i=1}^t \|g_{\xi_i}\|^2}}%}_{Private-Term}
\end{align}
where we write $g_{\xi_t}=\nabla L(\theta_t;z_{{\xi_{t}}})$. For simplicity, one might think about the one-dimension problem and set $b_0=0$. Note that the privacy mechanism different from Algorithm \ref{alg:privacy} because of the term $\frac{g_{\xi_t}+c_t}{\sqrt{b_0^2+\sum_{i=1}^t \|g_{\xi_i}\|^2}}$, compare to the term $g_{\xi_t}+c_t$ in Algorithm \ref{alg:privacy}. 

Our privacy mechanism is for some $b>0$ 
\begin{align}
    \mathcal{M}(x)= {f(x)+Z}
\end{align}
\begin{align}
    \mathcal{M}(x)=\frac{f(x)+Z}{\sqrt{b^2+\|f(x)\|^2}} \text{ where } Z\sim\mathcal{N}(0,\sigma_z^2I) \label{eq:machanism}
\end{align}
For simplification, let use only consider $d=1$.
%Compute the distribution of privacy loss random variable
\begin{defn}\label{def:privacy}
Suppose the privacy mechanism $\mathcal{M}:\mathbb{R}\to\mathbb{R}$ for some $f$ and $b>0$ follows
\[\mathcal{M}(x)=\frac{f(x)+Z}{\sqrt{b^2+f(x)^2}} \text{ where } Z\sim\mathcal{N}(0,\sigma_z^2) \]
Let the density function of $\mathcal{M}(x)$ be $f_{\mathcal{M}(x)}(y)$.
Define the privacy loss function $\mathcal{L}_{\mathcal{M}}^{x,x'}(y)$ and privacy loss random variable  $L_{\mathcal{M}}^{x,x'}$ as follows
\begin{align}
\mathcal{L}_{\mathcal{M}}^{x,x'}(y) &=\ln\left( \frac{f_{\mathcal{M}(x)}(y)}{f_{\mathcal{M}(x')}(y)} \right) \label{eq:privacy-def}; \quad  L_{\mathcal{M}}^{x,x'}= \mathcal{L}_{\mathcal{M}}^{x,x'}( \mathcal{M}(x)). 
\end{align}
\end{defn}
\me{The following theorem is for $f(x)=0$. Need to extend it more generally.}
\begin{thm}
Consider the privacy mechanism in Definition \ref{def:privacy}. The mechasism is $(\varepsilon,\delta)$-differentially private if 
\begin{align}
    \varepsilon    &= \frac{1}{\sigma_z^2} \left(1+\frac{b^2}{2(1 + \sqrt{1 + b^2})}\right) + \ln \left(\frac{1}{\delta} \right) \left(\frac{b}{b^2 +1}\right)^2 \sigma_z^2 \label{eq:privacy-thm}
\end{align}
\end{thm}
Let us interpret \eqref{eq:privacy-thm}. Observe if $b\gg 1$,
\begin{align}
    \varepsilon 
        = \frac{1}{\sigma_z^2}\Theta\left(b \right) + \ln \left(\frac{1}{\delta} \right)  \sigma_z^2 \Theta \left(\frac{1}{b^2}\right)  =\Theta \left( \frac{b}{\sigma_z^2} \right) 
\end{align}
We compare it with Gaussian mechanism  $\mathcal{M}_G(x)={f(x)+Z}$, which is $(\varepsilon,\delta)$-differentially private when 
\begin{align}
     \varepsilon = \frac{2\sqrt{\ln(1/\delta)}}{ \sigma_z},
\end{align}
For large $b$, the privacy of our mechanism can be amplified by the square $\sigma_z$ while  Gaussian mechanism is only linearly dependent on $\sigma$. However, whether our mechanism is better than  Gaussian depends on whether 
\begin{align}
     \frac{b}{\sigma_z}\leq  2\sqrt{\ln(1/\delta)}.
\end{align}

Note also that $b$ here is analogue to the stepsize  $1/\eta_t$ in Algorithm \ref{alg:privacy}. Thus our mechanism in  Algorithm \ref{alg:privacy-ada} depends implicitly on stepsize while Gaussian Mechanism in  Algorithm \ref{alg:privacy} is independent of of stepsize.

\begin{remark}
We note that we obtain optimality of privacy in \eqref{eq:privacy-thm} when the two terms on the right-hand side above are equals:
\begin{align}
   &\frac{1}{\sigma_z^2} \left(1+\frac{b^2}{2(1 + \sqrt{1 + b^2})}\right) = \ln \left(\frac{1}{\delta} \right) \left(\frac{b}{b^2 +1}\right)^2 \sigma_z^2  \\
\Leftrightarrow
  & \quad  \sigma_z = \frac{1}{\left(\ln({1}/{\delta})\right)^{1/4}}\left(1+\frac{b^2}{2(1 + \sqrt{1 + b^2})}\right)^{1/4}\left(\frac{b^2 +1}{b}\right)^{1/2} 
\end{align}
and the relationship between $b$ and $\varepsilon$ is
\begin{align}
    \varepsilon
        &\geq \left(\frac{b}{b^2 +1}\right)^2\sqrt{\ln \left(\frac{1}{\delta} \right) \left(1+\frac{b^2}{2(1 + \sqrt{1 + b^2})}\right)} = {\Theta}\left(\frac{1}{b^{3/2}}\sqrt{\ln \left(\frac{1}{\delta} \right)}\right)    
\end{align}

\end{remark}
The proof is given in Appendix 
% \input{privacy-guarantee-proof.tex}

%\me{not sure if this is a right way to understand the privacy if we only look at line 3 in Algorithm 2. Then we will have the same privacy guarantee as SGD.}

 
% \begin{align*}
% \exp(\frac{\alpha^2}{\sigma^2} - \varepsilon \alpha) &\geq \delta \\
% -\left ( \frac{\alpha^2}{\sigma^2} - \varepsilon \alpha\right) &\geq \ln \left( \frac{1}{\delta}\right) \\
% \alpha &= \sigma \sqrt{2\ln(\frac{1}{\delta})}
% \end{align*}


% \subsubsection{Attempt: Privacy Guarantee for Algorithm \ref{alg:privacy-ada}}
% The proof for this section follow the tutorial given in \url{https://simons.berkeley.edu/talks/large-scale-private-learning}.
% \me{Amplification by iteration}Observe the update of Algorithm  \ref{alg:privacy-ada} (AdaGrad) is 
% \begin{align}
%     \theta_{t+1}=\theta_t-\eta\frac{G_t}{\sqrt{b_0^2+\sum_{i=1}^t \|G_{i}\|^2}}=\theta_{t-1}-\eta \frac{g_{\xi_t}+c_t}{\sqrt{b_0^2+\sum_{i=1}^t \|g_{\xi_i}+c_i\|^2}}%}_{Private-Term}
% \end{align}
% where we write $g_{\xi_t}=\nabla L(\theta_t;z_{{\xi_{t}}})$. For simplicity, one might think about the one-dimension problem and set $b_0=0$. Note that the privacy mechanism does not follow Gaussian distribution because of the term $\frac{g_{\xi_t}+c_t}{\sqrt{b_0^2+\sum_{i=1}^t \|g_{\xi_i}+c_i\|^2}}$, compare to the term $g_{\xi_t}+c_t$ in Algorithm \ref{alg:privacy}. Our privacy mechanism is for some $b>0$ 
% \begin{align}
%     \mathcal{M}(x)=\frac{f(x)+Z}{\sqrt{b^2+\|f(x)+Z\|^2}} \text{ where } Z\sim\mathcal{N}(0,\sigma^2I) \label{eq:machanism}
% \end{align}

% %\me{not sure if this is a right way to understand the privacy if we only look at line 3 in Algorithm 2. Then we will have the same privacy guarantee as SGD.}

% \paragraph{Compute the distribution of privacy loss random variable}
% For simplification, let use only consider $d=1$ and define the density function of $\mathcal{M}$ as $f_{\mathcal{M}(x)}(y)$ for some $a$ and $b>0$
% \[\mathcal{M}(x)=\frac{f(x)+Z}{\sqrt{b^2+(f(x)+Z)^2}} \text{ where } Z\sim\mathcal{N}(0,\sigma^2) \]
% Define the privacy loss function for 
% \begin{align}
% L_{\mathcal{M}}^{x,x'} &=\log \left( \frac{f_{\mathcal{M}(x)}(y)}{f_{\mathcal{M}(x')}(y)} \right) \label{eq:privacy-def}\end{align}
% We work on the density function $f_{\mathcal{M}(x)}(y)$. Observe the inverse function of $\mathcal{M}(x)$ is \[Z = v(\mathcal{M}(x))= -f(x)+\frac{b|\mathcal{M}(x)|}{\sqrt{(1 - \mathcal{M}(x)^2)}} \text { with } -1< \mathcal{M}(x)<1.\footnote{There are two inverse functions $v(\mathcal{M}(x))= -f(x)\pm \frac{\sqrt{b}\mathcal{M}(x)}{(1 - \mathcal{M}(x)^2)}$. WOLG, we pick one of them}   \]
% The density of $\mathcal{M}(x)$ is
% \[f_{\mathcal{M}(x)}(y)=f_{X}(v(y))v'(y)	\propto\exp\left(-\frac{1}{2\sigma^2}\left( \frac{by}{(1 - y^2)}-a\right)^2 \right)\frac{b (1 + y^2))}{(1 - y^2)^2}
% \]
% Plugging it back to \eqref{eq:privacy-def}, we simplify $Z_{\mathcal{M}}^{d,d'}$
% \begin{align}
% Z_{\mathcal{M}}^{d,d'}
% &=\log \left(\frac{v(d)}{v(d')} \exp \left(- \frac{(v(d)-a)^2- (v(d')-a)^2}{2\sigma^2}\right)\right)  \\
% &=- \frac{(v(d)-a)^2- (v(d')-a)^2}{2\sigma^2} + \log \left(\frac{v(d)}{v(d')}\right) \label{eq:privacy-loss}
% \end{align}

% \paragraph{Compute $\mathbb{P}[Z_{\mathcal{M}}^{d,d'}\geq \varepsilon]\leq \delta$}
% \begin{lemma}
% A mechanism $\mathcal{M}:\mathcal{X}\to \mathcal{Y}$ is $(\varepsilon, \delta)-DP$ if for any $x,x'\in \mathcal{X}$, we have 
% $\mathbb{P}[Z_{\mathcal{M}}^{d,d'}\geq \varepsilon]\leq \delta$.
% \end{lemma}
% We need to work on for any $\alpha>0$:
% \begin{align}
% \mathbb{P} \left(Z_{\mathcal{M}}^{d,d'}\geq \varepsilon \right) &=\mathbb{P} \left(\exp\left(\alpha Z_{\mathcal{M}}^{d,d'}\right) \geq \exp\left(\alpha\varepsilon\right) \right)
% \leq \mathbb{E}\left[\exp\left(\alpha Z_{\mathcal{M}}^{d,d'}\right)\right]/\exp(\alpha \varepsilon) 
% %\\&= \mathbb{E}\left[\exp\left(\alpha Z_{\mathcal{M}}^{d,d'}(x)\right)\right]/\exp(\alpha \varepsilon)  \\
% \end{align}
% Using \eqref{eq:privacy-loss}, we get
% \begin{align}
%  \mathbb{E}\left[\exp\left(\alpha Z_{\mathcal{M}}^{d,d'}\right)\right]
%  = \mathbb{E}\left[  \left(\frac{v(d)}{v(d')}\right)^{\alpha}\exp \left(- \frac{\alpha(v(d)-a)^2- \alpha(v(d')-a)^2}{2\sigma^2}\right)\right]
% \end{align}

% \me{Need to type it down from the Jam Board. @Irina, could you help with this?}






==> olds/privacy_decreasing_sigma.tex <==
\section{Privacy Guarantee for Algorithm 2 when Decreasing the Noise Level}



Let us extend the analysis of the privacy of Algorithm 2, by considering the case in which the noise level $\sigma$ (which appears when drawing the random variable $c_t \sim \mathcal{N}(0, \sigma I)$) is monotonically decreasing. Let us assume that, at each iteration $t$ of Algorithm 2, we draw $c_t \sim \mathcal{N}(0, \sigma_t I)$, where

$$\sigma_t = \frac{\sigma}{t}, $$

\noindent for some fixed $\sigma >0$. Furthermore, let us consider that the stepsize $\eta_t$ is chosen as follows

$$ \eta_t =\frac{1}{\sqrt{t}}. $$


\noindent At each iteration $t$, the privacy of Algorithm 2 is embedded in the main variable of interest - $\theta_t$ - which is normally distributed with variance equal to 
    
    $$\mbox{Var}(\theta_t) = \eta_t^2 \sigma_t = \frac{1}{t} \cdot \frac{\sigma}{t} = \frac{\sigma}{t^2}.$$

\noindent Let $n$ be the batch size in Algorithm 2. Fix a (small) $\delta >0$. Then, by applying the privacy amplification by subsampling idea, we have that, at each iteration $t$, Algorithm 2 satisfies $(\epsilon_t, \delta)$ approximate differential privacy, where

$$ \epsilon_t = \frac{\sqrt{\log(1/\delta)}}{n\sigma_t}. $$

\noindent We would now like to obtain the "overall" differential privacy of Algorithm 2, after all of its $T$ execution steps are concluded. We can easily obtain this by invoking Theorem~\ref{thm:advanced-comp}. This stronger version of the "Advanced Composition Theorem" tells us that the differential privacy at the  conclusion of Algorithm 2 is characterized by

$$(\epsilon, \delta) = \left(\sqrt{(\sum_{t=1}^{T}\epsilon_t^2)\log(1/\delta)}, \delta\right).$$

\noindent In the above expression, we plug in the value of $\epsilon_t = \frac{\sqrt{\log(1/\delta)}}{n\sigma_t}$, and obtain that, in the final algorithm step, the privacy is characterized by the following $\epsilon$ parameter


\begin{align*}
 \epsilon = O\left( \sqrt{\sum_{t=1}^T \epsilon_t^2 \log(1/\delta)}\right) = O\left( \sqrt{\sum_{t=1}^T \frac{\log(1/\delta)}{n^2 \sigma_t^2}\log(1/\delta)}\right) =
 O\left( \sqrt{\sum_{t=1}^T \frac{\log(1/\delta)^2}{n^2 \sigma^2}} \cdot t\right) = O\left( \frac{\log(1/\delta)}{n \sigma} \sqrt{\frac{T(T+1)}{2}}\right). 
\end{align*}

\noindent The parameter $\epsilon$ controls the differential privacy guarantees of the Algorithm, with smaller values of $\epsilon$ implying \textit{stronger} differential privacy. To this end, we want to ensure $\epsilon = O(1)$ and for this to happen we need to impose the following condition on the total number of iterations $T$:

$$T \leq n.  $$

Let us now explore how this condition would change if we make a small small modification in the noise level. Namely, let us assume that, at each iteration, the monotonically decreasing noise is given by


$$ \sigma_t = \frac{\sigma}{t^p},$$

\noindent where $p < \frac{1}{2}$. By repeating the steps in the privacy analysis above, we obtain that the differential privacy at the final step $T$ of Algorithm 2 is characterized by

$$\epsilon = O\left( \sqrt{\sum_{t=1}^T t^p \frac{\log^2(1/\delta)}{n^2 \sigma^2}}\right) = O\left( \frac{\log(1/\delta)}{n\sigma} \sqrt{\int_{0}^T t^p dt}\right)= O\left( \frac{\log(1/\delta)}{n\sigma} \frac{T^{(p+1)/2}}{(p+1)/2}\right), $$

\noindent which implies that, in order to ensure that $\epsilon = O(1)$ (and, thus, have satisfactory differential privacy levels), we need to impose the following on $T$:

$$T \leq n^{2/(p+1)}.  $$

==> table1-best.tex <==

\begin{table}[tb]
%\vspace{-0.26cm}
\caption{\small \textbf{Mean accuracy of ADP-SGD/DP-SGD with polynomially decaying stepsizes.} This table reports \emph{Accuracy} for CIFAR10 with the mean and the corresponding standard deviation over five independent runs given a pair of $(\bar{\varepsilon},C_G,T, \text{Alg})$. The difference  (``Gap") between DP-SGDand ADP-SGDis provided for visualization purpose.  The results suggest that the more iterations or epochs we use, the more improvements ADP-SGD can potentially gain over DP-SGD. The results are reported in percentage ($\%$). The bolded number is the best accuracy in a row among epoch 60, 120 and 200 for the same gradient clipping $C_G$. See paragraph \textbf{Datasets and models} for detailed implementation.
% \becca{this needs elaboration. What is the objective function? How is accuracy measured? CIFAR-10?  MNIST? Not clear. }
% \becca{why do you sometimes indicate $\overline{\varepsilon}$ and sometimes $\varepsilon_T/C_\varepsilon$? It's a little hard for readers to keep track of all the different versions.}
} \label{table:cifar-decay}
\scalebox{0.65}{ 
\begin{tabular}{l|l|ccc|ccc|ccc}
\hline
\multirow{2}{*}{$\bar{\varepsilon}$}  & \multirow{2}{*}{Alg}   & \multicolumn{3}{c}{Gradient clipping $C_G=0.5$}       & \multicolumn{3}{c}{Gradient clipping $C_G=1.0$}   & \multicolumn{3}{c}{Gradient clipping $C_G=2.5/5.0$}       \\
                  &               & epoch=$60     $ & epoch$=120    $ & epoch$=200$& epoch=$60     $ & epoch$=120    $ & epoch$=200$ & epoch=$60     $ & epoch$=120    $ & epoch$=200$  \\ \hline\hline
\multirow{3}{*}{0.8} & ADPSGD & $55.46 \pm 0.561$& $\mathbf{57.31} \pm 0.134$& $57.02 \pm 0.375$& $56.11 \pm 0.130$& $52.97 \pm 0.804$& $47.94 \pm 1.024$& $37.91 \pm 1.976$& $24.4 \pm 3.055$& $11.13 \pm 0.895$\\ 
 & DPSGD & $55.71 \pm 0.300$& $\mathbf{56.75} \pm 0.572$& $56.13 \pm 0.588$& $56.03 \pm 1.004$& $52.54 \pm 0.979$& $44.33 \pm 0.624$& $37.73 \pm 0.800$& $20.73 \pm 2.856$& $10.23 \pm 0.033$\\ 
 & Gap& $-0.25$& $0.56$& $0.89$& $0.08$& $0.43$& $3.61$& $0.18$& $3.67$&N/A\\ \hline 
\multirow{3}{*}{1.2} & ADPSGD & $56.6 \pm 0.391$& $59.01 \pm 0.411$& $59.81 \pm 0.432$& $\mathbf{60.22} \pm 0.330$& $60.08 \pm 0.355$& $57.91 \pm 0.447$& $54.91 \pm 0.073$& $44.24 \pm 0.540$& $33.21 \pm 0.370$\\ 
 & DPSGD & $55.94 \pm 0.991$& $58.97 \pm 0.369$& $\mathbf{60.19} \pm 0.809$& $59.95 \pm 0.406$& $59.84 \pm 0.164$& $57.39 \pm 0.561$& $55.35 \pm 0.427$& $42.96 \pm 0.646$& $31.54 \pm 2.275$\\ 
 & Gap& $0.66$& $0.04$& $-0.38$& $0.27$& $0.24$& $0.52$& $-0.44$& $1.28$& $1.67$\\ \hline 
\multirow{3}{*}{1.6} & ADPSGD & $57.64 \pm 0.073$& $59.61 \pm 0.387$& $60.07 \pm 0.209$& $61.22 \pm 0.160$& $\mathbf{61.93} \pm 0.406$& $61.78 \pm 0.495$& $60.73 \pm 0.269$& $56.19 \pm 0.557$& $49.63 \pm 0.519$\\ 
 & DPSGD & $56.36 \pm 0.288$& $59.0 \pm 0.617$& $61.49 \pm 0.195$& $61.16 \pm 0.169$& $\mathbf{61.78} \pm 0.365$& $61.38 \pm 0.506$& $61.7 \pm 0.500$& $55.49 \pm 0.314$& $46.4 \pm 0.375$\\ 
 & Gap& $1.28$& $0.61$& $-1.42$& $0.06$& $0.15$& $0.4$& $-0.97$& $0.7$& $3.23$\\ \hline 
\multirow{3}{*}{3.2} & ADPSGD & $57.16 \pm 1.176$& $59.78 \pm 0.274$& $61.58 \pm 0.318$& $61.67 \pm 0.525$& $64.24 \pm 0.287$& $65.45 \pm 0.016$& $65.47 \pm 0.0$& $\mathbf{66.31} \pm 0.118$& $65.48 \pm 0.155$\\ 
 & DPSGD & $57.7 \pm 0.192$& $60.16 \pm 0.099$& $61.73 \pm 0.146$& $61.9 \pm 0.209$& $63.81 \pm 0.303$& $65.05 \pm 0.328$& $\mathbf{66.03} \pm 0.149$& $65.68 \pm 0.313$& $65.1 \pm 0.044$\\ 
 & Gap& $-0.54$& $-0.38$& $-0.15$& $-0.23$& $0.43$& $0.4$& $-0.56$& $0.63$& $0.38$\\ \hline 
\multirow{3}{*}{6.4} & ADPSGD & $58.05 \pm 0.275$& $60.01 \pm 0.276$& $61.66 \pm 0.380$& $62.16 \pm 0.274$& $64.5 \pm 0.524$& $65.64 \pm 0.256$& $67.3 \pm 0.049$& $68.65 \pm 0.026$& $\mathbf{69.45} \pm 0.134$\\ 
 & DPSGD & $56.74 \pm 0.589$& $59.79 \pm 0.802$& $61.83 \pm 0.394$& $61.99 \pm 0.241$& $64.58 \pm 0.155$& $65.81 \pm 0.206$& $66.97 \pm 0.217$& $68.36 \pm 0.282$& $\mathbf{69.18} \pm 0.166$\\ 
 & Gap& $1.31$& $0.22$& $-0.17$& $0.17$& $-0.08$& $-0.17$& $0.33$& $0.29$& $0.27$\\ \hline 
\end{tabular}}
%\vspace{-0.26cm}
\end{table}



% %\vspace{-0.26cm}
% % \me{put figure here}
% \begin{figure*}[tb]
% \includegraphics[width=0.245\linewidth]{./main-figs/}
% \includegraphics[width=0.245\linewidth]{./main-figs/beta10_epsilon-12_c-10_epoch-60_howmany_3_2.png}
% \includegraphics[width=0.245\linewidth]{./main-figs/beta10_epsilon-16_c-10_epoch-120_howmany_4_4.png}
% % \includegraphics[width=0.32\linewidth]{main-figs/mean_compare_epsilon-32_c-10_epoch-120.png}
% \includegraphics[width=0.245\linewidth]{./main-figs/mean_compare_epsilon-32_c-10_epoch-200_beta10.png}
% \includegraphics[width=0.245\linewidth]{./main-figs/beta25_epsilon-08_c-10_epoch-60_howmany_4_5.png}
% \includegraphics[width=0.245\linewidth]{./main-figs/beta25_epsilon-12_c-10_epoch-60_howmany_5_4.png}
% \includegraphics[width=0.245\linewidth]{./main-figs/beta25_epsilon-16_c-10_epoch-120_howmany_3_4.png}
% % \includegraphics[width=0.245\linewidth]{main-figs/beta25_epsilon-32_c-10_epoch-120_howmany_4_3.png}
% \includegraphics[width=0.245\linewidth]{./main-figs/mean_compare_epsilon-32_c-10_epoch-200_howmany_2_3.png}

% %\vspace{-0.15cm}
% % \includegraphics[width=0.32\linewidth]{main-figs/mean_compare_epsilon-32_c-10_epoch-120.png}
% \end{figure*}


==> table1-last.tex <==

\begin{table}[tb]
%\vspace{-0.26cm}
\caption{\small \textbf{Mean accuracy of ADP-SGD/DP-SGD with polynomially decaying stepsizes.} This table reports \emph{Accuracy} for CIFAR10 with the mean and the corresponding standard deviation over five independent runs given a pair of $(\bar{\varepsilon},C_G,T, \text{Alg})$. The difference  (``Gap") between DP-SGDand ADP-SGDis provided for visualization purpose.  The results suggest that the more iterations or epochs we use, the more improvements ADP-SGD can potentially gain over DP-SGD. The results are reported in percentage ($\%$). The bolded number is the best accuracy in a row among epoch 60, 120 and 200 for the same gradient clipping $C_G$. See paragraph \textbf{Datasets and models} for detailed implementation.
% \becca{this needs elaboration. What is the objective function? How is accuracy measured? CIFAR-10?  MNIST? Not clear. }
% \becca{why do you sometimes indicate $\overline{\varepsilon}$ and sometimes $\varepsilon_T/C_\varepsilon$? It's a little hard for readers to keep track of all the different versions.}
} \label{table:cifar-decay}
\scalebox{0.8}{ 
\begin{tabular}{l|l|ccc}
\hline
\multirow{2}{*}{$\bar{\varepsilon}$}  & \multirow{2}{*}{Alg}   & \multicolumn{3}{c}{Gradient clipping $C_G=1.0$}             \\
                  &               & epoch=$60     $ & epoch$=120    $ & epoch$=200    $\\ \hline\hline
\multirow{3}{*}{0.8}      & ADP          & $\mathbf{56.38} \pm 0.092  $ & $54.20 \pm 0.730  $ & $51.71 \pm 1.092  $   \\
                  & DP          & $\mathbf{56.13} \pm 0.909  $ & $52.72 \pm 0.938  $ & $44.68 \pm 0.576  $ \\
                  &	Gap	&	$	0.33	$&$	1.48	$&$	7.03	$\\\hline
\multirow{3}{*}{1.2}      & ADP          & $\mathbf{60.26} \pm 0.319  $ & $60.24 \pm 0.365  $ & $58.68 \pm 0.505  $ \\
                  & DP          & $\mathbf{60.09} \pm 0.330  $ & $60.02 \pm 0.204  $ & $57.56 \pm 0.514  $  \\
&	Gap	&	$	0.17	$&$	0.22	$&$	1.12	$\\ \hline                  
\multirow{3}{*}{1.6}       & ADP          & $61.30 \pm 0.219  $ & $\mathbf{61.98} \pm 0.420  $ & $61.88 \pm 0.507  $  \\
                  & DP          & $61.18 \pm 0.195  $ & $\mathbf{61.89} \pm 0.317  $ & $61.46 \pm 0.490  $  \\
&	Gap	&	$	0.12	$&$	0.09	$&$	0.42	$\\ \hline                  
\multirow{3}{*}{3.2}      & ADP          & $61.76 \pm 0.490  $ & $64.27 \pm 0.337  $ & $\mathbf{65.54} \pm 0.066  $ \\
                  & DP          & $62.02 \pm 0.248  $ & $63.88 \pm 0.275  $ & $\mathbf{65.11} \pm 0.339  $ \\
&	Gap	&	$	-0.26	$&$	0.39	$&$	0.43	$\\ \hline                  
\multirow{3}{*}{6.4}      & ADP          & $62.2 \pm 0.270   $ & $64.57 \pm 0.515  $ & $\mathbf{65.74} \pm 0.270  $  \\
                  & DP          & $62.06 \pm 0.244  $ & $64.61 \pm 0.180  $ & $\mathbf{65.84} \pm 0.206  $ \\ 
                  &	Gap	&	$	0.14	$&$	-0.04	$&$	-0.1	$\\ \hline
\end{tabular}}
% %\vspace{1.2cm}
\scalebox{0.8}{ \begin{tabular}{l|l|ccc}
\hline
\multirow{2}{*}{$\bar{\varepsilon}$}  & \multirow{2}{*}{Alg}     & \multicolumn{3}{c}{Gradient clipping $C_G=2.5$}             \\
                  &               & epoch=$60     $ & epoch$=120    $ & epoch$=200    $ \\ \hline\hline
\multirow{3}{*}{0.8}      & ADP          & $\mathbf{48.61} \pm 1.003  $ & $44.11 \pm 1.097  $ & $39.92 \pm 0.284 $ \\
                  & DP          & $\mathbf{38.06} \pm 1.029  $ & $23.64 \pm 0.796  $ & $17.75 \pm 1.068 $ \\
                  &	Gap	&$	10.55	$&$	20.47	$&$	22.17	$\\\hline
\multirow{3}{*}{1.2}      & ADP           & $\mathbf{56.63} \pm 0.308  $ & $52.26 \pm 0.328  $ & $50.7 \pm 1.038  $ \\
                  & DP          & $\mathbf{55.71} \pm 0.418  $ & $43.16 \pm 0.604  $ & $32.00 \pm 2.281 $ \\
&	Gap	&$	0.92	$&$	9.1	$&$	18.7	$\\ \hline                  
\multirow{3}{*}{1.6}       & ADP        & $\mathbf{61.52} \pm 0.313  $ & $58.60 \pm 0.332  $ & $56.07 \pm 0.046 $ \\
                  & DP       & $\mathbf{61.76} \pm 0.334  $ & $55.68 \pm 0.243  $ & $46.74 \pm 0.428 $ \\
&	Gap	&$	-0.24	$&$	2.92	$&$	9.33	$\\ \hline                  
\multirow{3}{*}{3.2}      & ADP          & $65.34 \pm 0.12   $ & $\mathbf{66.41} \pm 0.054  $ & $65.74 \pm 0.106 $ \\
                  & DP       & $\mathbf{66.08 }\pm 0.130  $ & $65.73 \pm 0.333  $ & $65.17 \pm 0.115 $ \\
&	Gap&$	-0.44	$&$	0.68	$&$	0.57	$\\ \hline                  
\multirow{3}{*}{6.4}      & ADP          & $67.35 \pm 0.057  $ & $68.72 \pm 0.045  $ & $\mathbf{69.51} \pm 0.179 $ \\
                  & DP         & $67.06 \pm 0.244  $ & $68.46 \pm 0.321  $ & $\mathbf{69.28 }\pm 0.147 $\\ 
                  &	Gap&$	0.29	$&$	0.26	$&$	0.23	$\\ \hline
\end{tabular}}
%\vspace{-0.26cm}
\end{table}



% %\vspace{-0.26cm}
% % \me{put figure here}
% \begin{figure*}[tb]
% \includegraphics[width=0.245\linewidth]{./main-figs/}
% \includegraphics[width=0.245\linewidth]{./main-figs/beta10_epsilon-12_c-10_epoch-60_howmany_3_2.png}
% \includegraphics[width=0.245\linewidth]{./main-figs/beta10_epsilon-16_c-10_epoch-120_howmany_4_4.png}
% % \includegraphics[width=0.32\linewidth]{main-figs/mean_compare_epsilon-32_c-10_epoch-120.png}
% \includegraphics[width=0.245\linewidth]{./main-figs/mean_compare_epsilon-32_c-10_epoch-200_beta10.png}
% \includegraphics[width=0.245\linewidth]{./main-figs/beta25_epsilon-08_c-10_epoch-60_howmany_4_5.png}
% \includegraphics[width=0.245\linewidth]{./main-figs/beta25_epsilon-12_c-10_epoch-60_howmany_5_4.png}
% \includegraphics[width=0.245\linewidth]{./main-figs/beta25_epsilon-16_c-10_epoch-120_howmany_3_4.png}
% % \includegraphics[width=0.245\linewidth]{main-figs/beta25_epsilon-32_c-10_epoch-120_howmany_4_3.png}
% \includegraphics[width=0.245\linewidth]{./main-figs/mean_compare_epsilon-32_c-10_epoch-200_howmany_2_3.png}

% %\vspace{-0.15cm}
% % \includegraphics[width=0.32\linewidth]{main-figs/mean_compare_epsilon-32_c-10_epoch-120.png}
% \end{figure*}

\begin{figure}[htb]
\includegraphics[width=0.32\linewidth]{main-figs/beta1.0_epsilon-0.8_c-1.0_epoch-120_howmany_5_5.png} 
\includegraphics[width=0.32\linewidth]{main-figs/beta1.0_epsilon-3.2_c-1.0_epoch-200_howmany_4_3.png} 
% \includegraphics[width=0.32\linewidth]{main-figs/beta1.0_epsilon-0.8_c-1.0_epoch-120_howmany_5_5.png}
% \includegraphics[width=0.32\linewidth]{main-figs/beta1.0_epsilon-1.2_c-1.0_epoch-200_howmany_4_5.png}
\includegraphics[width=0.32\linewidth]{main-figs/beta1.0_epsilon-1.6_c-1.0_epoch-200_howmany_5_4.png}
\includegraphics[width=0.32\linewidth]{main-figs/beta2.5_epsilon-0.8_c-1.0_epoch-120_howmany_5_5.png} 
\includegraphics[width=0.32\linewidth]{main-figs/beta2.5_epsilon-1.6_c-1.0_epoch-200_howmany_3_3.png}
\includegraphics[width=0.32\linewidth]{main-figs/beta2.5_epsilon-3.2_c-1.0_epoch-200_howmany_2_3.png} 
% \includegraphics[width=0.32\linewidth]{main-figs/beta1.0_epsilon-6.4_c-1.0_epoch-200_howmany_4_3.png} 
% \includegraphics[width=0.32\linewidth]{main-figs/beta2.5_epsilon-6.4_c-1.0_epoch-200_howmany_3_4.png} 
\caption{\small  \textbf{Test accuracy with respect to iteration $t$ using ADP-SGD/DP-SGD with polynomially decaying stepsizes.} The black lines corresponding to the right y-axis are measured by the test accuracy on CIFAR10 for a CNN model using ADP-SGD  (solid line) and DP-SGD (dash line).   The shaded region is one standard deviation.  Each plot corresponds to a fixed $T$ (see x-axis) and a privacy budget $\bar{\varepsilon}$ with a fixed gradient clipping value $C_G$ (see title). The top (bottom) column is for gradient clipping $C_{G}=1.0$ ($2.5$). Same as \cref{fig:compare}, the monotone green curves, which correspond to the left vertical y-axis, show the actual noise for  $\alpha_t=1/\sqrt{\eta_t}$ (ADP-SGD, the solid line) and  $\alpha_t=1$ (DP-SGD, the dashed line).  Each plot, the best mean accuracy among the iterations are included in Table \ref{table:cifar-decay}. %The top/bottom rows from 1st to 4th column correspond to the privacy budgets from $0.8$ (epoch 60), $1.2$ (epoch 60), $1.6$ (epoch 120), and $3.2$ (epoch 200).  
% \becca{the color scheme is confusing here. for noise, they're both green, but for accuracy, there's a mix of orange and blue. I think both noise plots should be the same color (e.g. green) and both accuracy plots should be the same color (e.g. blue)}
% \becca{I cannot tell how the top and bottom rows are different}
% \becca{What is the objective? How is accuracy measured?}
}\label{fig:cifar-decay}
%\vspace{-0.36cm}
\end{figure}

==> zfigure1.tex <==

\begin{figure}[H]
\includegraphics[width=0.32\linewidth]{figs/figs-120/mean_compare_epsilon-1.6_c-0.1_epoch-200_howmany_4_2.png}
\includegraphics[width=0.32\linewidth]{figs/figs-120/mean_compare_epsilon-1.6_c-0.5_epoch-200_howmany_5_5.png}
\includegraphics[width=0.32\linewidth]{figs/figs-120/mean_compare_epsilon-1.6_c-1.0_epoch-200_howmany_3_4.png}
\includegraphics[width=0.32\linewidth]{figs/figs-120/mean_compare_epsilon-3.2_c-0.1_epoch-200_howmany_3_2.png}
\includegraphics[width=0.32\linewidth]{figs/figs-120/mean_compare_epsilon-3.2_c-0.5_epoch-200_howmany_4_5.png}
\includegraphics[width=0.32\linewidth]{figs/figs-120/mean_compare_epsilon-3.2_c-1.0_epoch-200_howmany_3_3.png}
\includegraphics[width=0.32\linewidth]{figs/figs-120/mean_compare_epsilon-6.4_c-0.01_epoch-200_howmany_3_2.png}
\includegraphics[width=0.32\linewidth]{figs/figs-120/mean_compare_epsilon-6.4_c-0.1_epoch-200_howmany_5_4.png}
\includegraphics[width=0.32\linewidth]{figs/figs-120/mean_compare_epsilon-6.4_c-1.0_epoch-200_howmany_3_4.png}

\includegraphics[width=0.32\linewidth]{figs/figs-120/mean_compare_epsilon-12.8_c-0.01_epoch-200_howmany_3_4.png}
\includegraphics[width=0.32\linewidth]{figs/figs-120/mean_compare_epsilon-12.8_c-0.1_epoch-200_howmany_5_5.png}
\includegraphics[width=0.32\linewidth]{figs/figs-120/mean_compare_epsilon-12.8_c-1.0_epoch-200_howmany_3_4.png}

   \caption{ {\small\textbf{ADP-SGD v.s. DP-SGD with decreasing stepsizes $\eta/b_t=1/\sqrt{20+ct}$ for Epoch 200.}  Each plot corresponds to a hyper-parameter  $c$ and a privacy budget $\varepsilon$ (see title). The shaded orange and light-blue curves, corresponding to the left vertical axis, show the averaged test error for DP-SGD (dash line) and ADP-SGD (solid line). The shaded region is one standard deviation. Same as \cref{fig:compare}, the monotone blue solid and dash curves corresponding to the right vertical axis show the overall privacy for $\alpha_t=1$ (DP-SGD), represented by the dashed line, and $\alpha_t=1/\sqrt{\eta_t}$ (ADP-SGD), represented by the  solid line. From 1st to 4th row, it describes the privacy budgets from $1.6$, $3.2$, $6.4$ and $12.8$.}}\label{fig:epoch-200}
\end{figure}


\begin{figure}[H]
\includegraphics[width=0.32\linewidth]{figs/figs-60/mean_compare_epsilon-1.6_c-0.1_epoch-60_howmany_6_6.png}
\includegraphics[width=0.32\linewidth]{figs/figs-60/mean_compare_epsilon-1.6_c-0.5_epoch-60_howmany_6_5.png}
\includegraphics[width=0.32\linewidth]{figs/figs-60/mean_compare_epsilon-1.6_c-2.0_epoch-60_howmany_4_3.png}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[width=0.32\linewidth]{figs/figs-60/mean_compare_epsilon-3.2_c-0.1_epoch-60_howmany_5_5.png}
\includegraphics[width=0.32\linewidth]{figs/figs-60/mean_compare_epsilon-3.2_c-0.5_epoch-60_howmany_5_6.png}
\includegraphics[width=0.32\linewidth]{figs/figs-60/mean_compare_epsilon-3.2_c-2.0_epoch-60_howmany_3_6.png}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\includegraphics[width=0.32\linewidth]{figs/figs-60/mean_compare_epsilon-6.4_c-0.001_epoch-60_howmany_4_6.png}
\includegraphics[width=0.32\linewidth]{figs/figs-60/mean_compare_epsilon-6.4_c-0.1_epoch-60_howmany_5_5.png}
\includegraphics[width=0.32\linewidth]{figs/figs-60/mean_compare_epsilon-6.4_c-1.0_epoch-60_howmany_6_6.png}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\includegraphics[width=0.32\linewidth]{figs/figs-60/mean_compare_epsilon-12.8_c-0.001_epoch-60_howmany_6_6.png}
\includegraphics[width=0.32\linewidth]{figs/figs-60/mean_compare_epsilon-12.8_c-0.1_epoch-60_howmany_6_5.png}
\includegraphics[width=0.32\linewidth]{figs/figs-60/mean_compare_epsilon-12.8_c-1.0_epoch-60_howmany_4_4.png}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \caption{ {\small\textbf{ADP-SGD v.s. DP-SGD with decreasing stepsizes $\eta/b_t=1/\sqrt{20+ct}$ for Epoch 60.}  Each plot corresponds to a hyper-parameter  $c$ and a privacy budget $\varepsilon$ (see title).  From 1st to 4th row, it describes the privacy budgets from $1.6$, $3.2$, $6.4$ and $12.8$. See \cref{fig:epoch-200} for the  detailed description. }}\label{fig:epoch-60}
\end{figure}
